ARMOR: Accelerating RTL Simulation by Mitigating the Front-End Bottleneck Using Node Compression

RTL simulation is indispensable in chip design. High-performance simulators typically lower each node in the RTL graph into an instruction sequence. Although this per-node lowering enables aggressive compiler optimizations, it dramatically increases the code footprint, severely exceeding instruction cache capacity and causing front-end bottlenecks. Our profiling reveals that over 50% of pipeline stalls are caused by the CPU front-end, becoming a key performance bottleneck in state-of-the-art RTL simulators. However, reaping the optimization benefits of fully unrolling the RTL graph while simultaneously reducing the code footprint to mitigate front-end bottlenecks remains highly challenging. In this paper, we propose ARMOR, an efficient RTL simulator designed to alleviate the front-end bottleneck through node compression. The key idea is to exploit the data parallelism exposed by the unrolling RTL graph and the insufficient bit-space utilization revealed by per-node lowering, leveraging bit-level data parallelism to compress multiple nodes simultaneously, so that a single instruction sequence can serve multiple nodes instead of one per node. To achieve profitable node compression, we first propose a module-aware isomorphic subgraph identification method that leverages structural isomorphism across module instances to systematically identify compression opportunities at the subgraph level. We then propose an alignment-aware dense packing strategy that groups nodes into packs according to dataflow dependencies while preserving data reuse, complemented by greedy merging strategies to enhance bit-space utilization. Finally, we implement a unified bit-level parallelism scheme to support bit-level parallel execution of compressed nodes. Experimental results show that ARMOR achieves 1.6x speedup on CPU designs and 2.7x speedup on AI accelerators compared to state-of-the-art simulators.

==> Section/ack.tex <==
\begin{acks}
   
\end{acks}


==> Section/challenge.tex <==

\subsection{Challenges in Node Compression}
\begin{figure*}[htbp]
    \centering
    \SetCaptionSpacing{0.10cm}{0.10cm}
    \includegraphics[width=0.9\linewidth]{Figure/motivation2_6.pdf}
    \caption{
        (a): Example of an RTL graph.
        % (b): suboptimal node grouping 产生2次data reorangement 开销。
        % (c): subgraph-level node grouping 产生1次 data reorangement 开销
        (b) Suboptimal node packing incurs two rounds of data rearrangement that permute operands to align with the expected computation pattern~(e.g., aligning operands of node 4). 
        (c) Subgraph-level packing reduces the overhead to one round.
    }
    \label{fig:challenge}
\end{figure*}

% Although isomorphic nodes within the same topological level can, in principle, share execution through node compression, poorly designed compression strategies may incur frequent data rearrangement, making compressed execution unprofitable. 
Although isomorphic nodes within the same topological level can, in principle, be executed collectively via node compression, poorly designed compression strategies may incur frequent data rearrangement, thus rendering compressed execution unprofitable.
Effective node compression thus faces several critical challenges:

% 钉子和锤子：目前的有类似的锤子，但是不好。
% \textbf{Challenge 1: Lack of a subgraph-level perspective.}\label{sec:challenge1}
\textbf{Challenge 1: Lack of subgraph-level coordination for node compression.}\label{sec:challenge1}
% node compression面临的第一个挑战是如何挖掘压缩机会。
% The first challenge of node compression is how to identify compression opportunities.
% 现有启发式方法通常依赖局部搜索策略，例如\textit{use-def}或\textit{def-use}链~\selfcite{PLDI_2000_Larsen,ASPLOS_2021_Chen}。在大量同构节点存在的情况下，局部策略容易被误导，因为可压缩节点被孤立处理，缺乏子图级的协调视角。这可能导致节点分组不合理，从而引发多轮数据重排，显著增加执行开销。因此如何高效识别同构子图来提供全局视角是pre-packing挑战。
Existing general-purpose heuristic approaches rely on local search strategies~\selfcite{PLDI_2000_Larsen, ASPLOS_2021_Chen, Shahbahrami2006, MICRO_2017_Huh, MICRO_2010_Barik}, such as \textit{use-def} or \textit{def-use} chains~\selfcite{PLDI_2000_Larsen}, to pack nodes. 
% In the presence of numerous isomorphic nodes, these local searches are easily misled~\selfcite{ASPLOS_2012_Park}, as compressible nodes are handled in isolation without a coordinated subgraph-level view. 
% This can lead to suboptimal node packing and multiple rounds of data rearrangement, increasing execution overhead. 
In scenarios with numerous isomorphic nodes, these local searches are easily misled~\selfcite{ASPLOS_2012_Park}, as compressible nodes are handled in isolation, lacking subgraph-level coordination. 
This can lead to suboptimal node packing and multiple rounds of data rearrangement, increasing overhead. 
% As shown in Figure~\selfref{fig:challenge}~(b), the suboptimal packing incurs two rounds of data rearrangement, resulting from forming packs \textit{G1} and \textit{G2} without accounting for \textit{G3}.
By comparing the original RTL graph in Figure~\selfref{fig:challenge}~(a) with the suboptimal packing in Figure~\selfref{fig:challenge}~(b), we observe that two rounds of data rearrangement occur due to forming packs \textit{G1} and \textit{G2} without considering \textit{G3}.
In contrast, the optimized packing in Figure~\selfref{fig:challenge}~(c) reduces this to a single round by leveraging isomorphic subgraphs.
Therefore, efficiently identifying isomorphic subgraphs to provide a subgraph-level coordination constitutes a fundamental pre-packing challenge.

\textbf{Challenge 2: Conflict between bit-space utilization and data reuse efficiency.}\label{sec:challenge2}
% 节点打包过程本质上涉及位空间利用率与数据复用效率之间的权衡关系。基于数据依赖的分组能够提升生产者–消费者局部性，从而减少数据移动开销，但可能导致机器字中存在未充分利用的位，降低整体利用率。相反，以提升位利用率为目标的打包策略则可能破坏数据局部性，引入额外的数据重排开销。由于两者优化目标相互制约，如何在保证高位利用率的同时维持高效的数据复用，构成了节点打包中的核心挑战。
Node packing involves a trade-off between \textit{bit-space utilization} and \textit{data reuse efficiency}. 
Packing nodes based on data dependencies improves data reuse between producers and consumers, thereby reducing data rearrangement overhead, but may leave bits within a machine word underutilized, lowering overall utilization. 
Conversely, packing strategies that aggressively maximize bit utilization may break data reuse and introduce frequent data rearrangement. 
As these objectives are inherently conflicting, achieving high bit-space utilization while maintaining high data reuse constitutes a fundamental challenge in node packing.
% As improving one objective inevitably degrades the other, jointly optimizing both remains a fundamental challenge in node packing.

\textbf{Challenge 3: Incompatibility between bit-level parallel execution and cross-\subwordTerm{} dependent operations.}\label{sec:challenge3}
% 节点压缩通过 bit-level 打包将多个节点映射到同一数据字，实现并行执行。然而，这种方式依赖各 bit（lane）之间相互独立的假设。
% 目前只有逻辑运算满足lane-independet,尽管RTL graph 逻辑运算的占比很高，另外一些常见的运算如eq运算，并不支持lane- independent。
% 因此，在保证 bit-level 并行性的前提下，如何支持非 lane-independent 运算，是压缩执行阶段的重大挑战。
% Node compression maps multiple nodes into a single machine word via bit-level packing to enable parallel execution. 
Node compression maps multiple nodes onto a single machine word to enable bit-level parallel execution, where each node is allocated a contiguous group of bits, referred to as a bit \textit{slice}.
However, this technique only applies to \subwordTerm{}-independent operations, such as logical operations; any cross-\subwordTerm{} dependencies would prevent correct execution.
For example, for equality comparisons, the final output is computed as
\(
R = \bigwedge_{l=0}^{L-1} \text{Eq}(X_l, Y_l),
\)
where \(X_l\) and \(Y_l\) are the operands of \subwordTerm{} \(l\), and \(L\) is the number of \subwordTerm s. 
Ideally, each \subwordTerm{} would produce an independent 0/1 result, but the cross-\subwordTerm{} dependency forces aggregation into a single output.
% While logic operations in the RTL graph generally satisfy this lane-independence property, other common operations, such as equality comparisons, do not. 
Consequently, supporting cross-\subwordTerm{} dependent operations while preserving bit-level parallelism remains a challenge in the compressed execution stage.

To overcome these challenges, we propose the \papertitle{} framework, which is introduced in the following sections.

% \subsection{Challenge of Node Compression}
% % 尽管同一拓扑层中的同构节点在理论上可以通过压缩方式实现共享执行，但在实际中，不友好的压缩方式会带来data rearrangement开销，使得压缩运算无利可图。高效的节点压缩仍面临多方面挑战。其根本原因在于，节点压缩不仅涉及结构等价性的识别，还涉及跨节点的数据布局优化以及压缩执行机制的协同设计。具体而言，主要存在以下三个方面的关键挑战：

% Although isomorphic nodes within the same topological level can, in principle, share execution through compression, poorly designed compression strategies may incur substantial data rearrangement overhead, making compressed execution unprofitable. 
% Therefore, achieving efficient node compression in practice is non-trivial, which faces three key challenges:


% % 挑战1:
% \textbf{Challenge 1: Lack of a global subgraph-level perspective.} Existing heuristic approaches rely on local search, such as \textit{use}-\textit{def} or \textit{def}-\textit{use} chains~\selfcite{PLDI_2000_Larsen,ASPLOS_2021_Chen}, and are prone to being misled in the presence of numerous isomorphic nodes~\selfcite{ASPLOS_2012_Park}, 
% due to compressible nodes are handled separately, lacking a holistic view of the subgraph for coordinated compression.
% As shown in Figure~\selfref{fig:challenge}~(b), the suboptimal grouping incurs two rounds of data reorganization, resulting from forming groups \textit{G1} and \textit{G2} without accounting for \textit{G3}.
% In contrast, the optimized grouping in Figure~\selfref{fig:challenge}~(c) reduces this overhead to a single round by leveraging isomorphic subgraphs.
% However, identifying isomorphic subgraphs is NP-hard~\selfcite{graph_iso1,graph_iso2}. 
% % 为了克服直接在RTL graph上识别同构子图的问题，我们利用RTL graph天然具备的结构同构性。具体而言，RTL graphs are not arbitrary structures, but are systematically generated from hardware architectures through module duplication.
% To overcome the difficulty of performing direct isomorphism identification on RTL graphs, we exploit the structural regularity inherent in RTL designs, especially for highly parallel designs~\selfcite{high_parallel_archi1,high_parallel_archi2,high_parallel_archi3}. 
% Specifically, RTL graphs are not arbitrary structures, but are systematically generated from hardware architectures via module duplication, which naturally results in structural isomorphism among instances of the same module.
% % 相同module的不同instance天然具备同构性，因此，By leveraging module hierarchy, we 能够高效实现同构子图识别 in the RTL graph.
% By leveraging the module hierarchy, we propose module-aware isomorphic subgraph identification method to efficiently identify isomorphic subgraphs in RTL graphs.

% % Modern highly parallel designs~\selfcite{high_parallel_archi1,high_parallel_archi2,high_parallel_archi3} typically replicate computation modules rather than constructing entirely unique logic structures.


% % 挑战2: bit-space利用率与数据复用效率的失配
% % data reuse efficientcy 关注的是数据流的依赖顺序（横向约束），而bit-space利用率关注的是在同一拓扑层中可并行节点之间的组合优化（纵向约束）。这种纵横约束意味仅从单一维度考虑pack是不可行的。具体而言，单纯依赖数据流进行打包可能导致后续 pack 无法充分填满，从而限制整体位空间利用率。而过度追求bit-space利用率导致压缩后的数据无法在生产者–消费者之间直接复用，引入频繁的数据重排开销。
% % We propose a two-pronged heuristic strategy that tackles both improve bit-space utilization and minimal data rearrangement. 我们的核心策略是，有限保证pack的连续性以减少数据重排开销，然后再使用合并策略逐步提高bit空间利用率。

% \textbf{Challenge 2: Mismatch between bit-space utilization and data reuse efficiency.} 
% Data reuse efficiency primarily concerns the dependency order of the data flow (horizontal constraints), whereas bit-space utilization focuses on the combinational optimization among parallelizable nodes within the same topological level (vertical constraints). 
% These orthogonal constraints imply that packing nodes based on a single dimension is insufficient. 
% Specifically, packing solely according to the data flow may leave subsequent packs underfilled, limiting overall bit-space utilization. Conversely, overly prioritizing bit-space utilization can prevent compressed data from being directly reused between producers and consumers, introducing frequent data rearrangement overhead.
% To address this challenge, we propose a two-pronged heuristic strategy that simultaneously improves bit-space utilization while minimizing data rearrangement. 
% The core idea is to first maintain continuity within each subgraph to reduce data reshuffling overhead, and then progressively enhance bit-space utilization through merging strategies.


% % 挑战3:\textbf{挑战三：bit-level 并行执行与跨位依赖语义的不一致。}  
% % 节点压缩通过bit-level打包将多个逻辑节点映射到同一数据字中，从而实现并行执行。然而，这种bit-level并行隐含了一个关键前提，即各bit之间相互独立（lane-independent）。该前提在逻辑运算（如AND、OR、XOR）中天然成立，但对于涉及跨位依赖的运算，则往往不再成立。具体而言，此类运算通常需要在多个bit之间进行归约或传播，从而破坏打包数据中的lane边界，导致不同节点之间发生语义干扰。因此，如何在保持bit-level并行性的同时，正确高效地支持非lane-independent运算，成为节点压缩执行阶段的核心挑战。
% % 为了解决这一挑战，我们提出一种面向非lane-independent运算的压缩执行变换策略。具体而言，通过对运算进行位级分解与重组，充分利用bit manipulation unit（BMU）对相关bit进行规约与传播，并结合查找表（lookup table, LUT）高效实现EQ等跨位依赖运算，从而保证了在bit-level打包下的运算语义正确性和执行效率。

% \textbf{Challenge 3: Incompatibility between bit-level parallel execution and cross-bit dependency semantics.}  
% Node compression maps multiple nodes into a single machine word via bit-level packing to enable parallel execution. 
% However, this approach relies on the key assumption that bits (lanes) are independent. 
% While this assumption holds naturally for logic operations, it breaks down for operations involving cross-bit dependencies. Such operations require reduction or propagation across multiple bits, which disrupts lane boundaries and leads to semantic interference among packed nodes. 
% Therefore, efficiently supporting non-lane-independent operations while preserving bit-level parallelism remains a critical challenge in compressed execution.
% To address this challenge, we propose a compression-execution transformation strategy for non-lane-independent operations. 
% Specifically, operations are decomposed and reorganized at the bit level, fully leveraging the bit manipulation unit (BMU) to reduce and propagate relevant bits. Cross-bit dependent operations, such as Eq operations, are efficiently implemented using lookup tables (LUTs). 
% This approach ensures both semantic correctness and execution efficiency under bit-level packed execution.



==> Section/challenge2_method_v1.tex <==

\subsection{Dependency-Aware Dense Packing} % Alignment-aware Packing
% 子图内部：最大化bit-space利用率
% 子图边界：repack
While compression domains identify structurally equivalent nodes across isomorphic subgraphs introduced by module instances, they do not directly correspond to hardware-executable units due to the limitation of machine word. 
To implement efficient packed execution, nodes within each domain must be organized into \emph{packs} that maximize bit-space utilization while minimizing the overhead of data rearrangement.
% 然而，获得最优的packs是NP-hard问题。
However, finding the optimal packing is NP-hard, as it generalizes classic bin packing and quadratic assignment problems.

% 为了解决该问题，我们采用
To address this problem, we employ a two-pronged heuristic strategy that tackles both improve bit-space utilization and minimal data rearrangement.
% 我们采用对齐感知打包（alignment-aware packing）方法。该方法的核心在于严格遵循节点间的数据流依赖关系，最大程度地减少运行时的数据重排开销。具体来说，算法通过依赖感知的方式扩展pack，使得上游节点产生的数据可以被下游节点直接消费。
To reduce data rearrangement overhead, we adopt the alignment-aware packing method. The core of this approach is to strictly follow the dataflow dependencies between packs, minimizing runtime data rearrangement overhead. Specifically, we expand packs in a dependency-aware manner, ensuring that data produced by upstream packs can be directly consumed by downstream packs.
% 为了进一步提升位宽空间利用率，我们在初始阶段对每个压缩域选择最大可行节点组（Max Feasible Group），尽可能填满一个机器字，从而保证每个初始化pack的bit space利用率。
% 此外，在打包完成后，对于同一压缩域内的多个pack，如果它们可以合并且总位宽不超过机器字限制，则将其合并。
To improve bit-space utilization, a maximal feasible group of nodes is first selected to fill a machine word as fully as possible, ensuring high initial bit-space efficiency.
After forming and expanding the initial packs, multiple packs within the same compression domain are merged whenever possible, provided that the total bit-width does not exceed the machine word size.
% 通过结合依赖感知的pack扩展与域内最大可行组打包及pack合并策略，alignment-aware packing 不仅保证了低运行时重排开销，同时显著提高了位宽空间利用率。
% 为了解决该问题，我们采用两阶段pack方法。首先，在每个子图内部，我们采用greedy方法来最大化bit-space利用率。
By combining dependency-aware pack expansion with maximal feasible group selection and intra-domain pack merging, dependency-aware packing not only low data reorganization overhead but also enhances bit-space utilization.





% 得益于我们能够高效地识别subgraph，因此，在partition compression domains时，我们遵循subgraph内部的dataflow依赖关系，这样能够保证在subgraph内部，pack的输出会直接被consumer，避免了packing/unpacking开销。
% By leveraging efficient subgraph identification, the partitioning strictly follows the subgraph’s internal dataflow, ensuring that \textit{pack} results are directly consumed within the subgraph and eliminating packing/unpacking overhead.
% 其次，由于子图边界可能存在结构差异，无法完全保持对齐。在这种情况下，我们的策略是对边界节点进行选择性重打包，避免影响后续分组。


% \subsection{Structurally Aligned Node Grouping}
% % \begin{figure*}[htbp]
% %     \centering
% %     \includegraphics[width=\linewidth]{Figure/node_align.pdf}
% %     \caption{
% %         xxx
% %     }
% %     \label{fig:node_align}
% % \end{figure*}
% % Goal:
% %     align and pack corresponding nodes across subgraphs
% % Output:
% %     execution groups

% % topology-based node grouping。 不同instance的上下文环境不同，如果全部grouping，则容易产生loop依赖。因此需要避免环依赖。

% % 确定运算的最大位宽：max（operands， results）
% % 

% While compression domains identify structurally equivalent nodes across isomorphic subgraphs introduced by module instances, they do not directly correspond to hardware-executable units. 
% To enable efficient packed execution, nodes within each domain must be organized into \emph{packs} that satisfy hardware constraints and minimize data reorganization overhead.
% % 具体而言，当压缩域的大小超过处理单元所支持的宽度时，我们需要划分压缩域为多个execution groups。不合理的划分会增加数据pack和unpack开销。如图xxx所示，假设压缩域大小为4，相同颜色表示，机器支持的execution group的大小为2。采用（a）的划分方法，使得G1和G3的运算结果需要先unpack然后再pack给G2和G4使用，而（b）的划分方法则不存在pack/unpack开销。
% Specifically, when the size of a compression domain exceeds the width supported by the processing elements, the domain must be partitioned into multiple packs. 


% A naive partitioning strategy may significantly increase data reorganization overhead. 
% As illustrated in Fig.~XXX, consider a compression domain of size four under a hardware execution width of two.
% Partitioning scheme (a) satisfies the width constraint but disrupts structural alignment across dependent domains. As a result, intermediate values must be unpacked and repacked when transferred between execution groups, introducing unnecessary overhead. 
% In contrast, scheme (b) preserves cross-domain alignment, allowing dependent operations to remain consistently grouped and eliminating additional pack/unpack operations.
% Therefore, execution group partitioning must account for dependency-aware structural alignment.

% % 除了通过 dependency-aware structural alignment 减少数据移动开销外，还必须同时考虑硬件利用效率。
% Beyond dependency-aware structural alignment for minimizing data movement overhead, hardware utilization efficiency must also be considered. 
% % 在某些情况下，若严格保持跨压缩域的结构对齐，会导致执行组未充分填满硬件执行单元的可用位宽，从而降低并行执行效率。
% % 如图~XXX 所示，在严格保持 dependency-aware structural alignment 的情况下，为了维持跨压缩域之间的组级对齐，多个压缩域可能被迫进行划分。虽然这种方式能够保持依赖关系在执行组层面的结构一致性，但会增加 execution group 的总数量，从而直接增加打包指令的发射次数。
% % 若在子图边界处进行 selective relaxation，允许适度打破跨域对齐关系，则每个压缩域可以作为更大粒度的 execution group 执行。尽管这种方式可能引入一定的数据移动开销，但由于 execution group 数量减少，整体指令数量随之下降。
% % 因此，执行组构建需要在依赖对齐带来的数据移动开销与 execution group 数量之间进行权衡
% As illustrated in Fig.~XXX, under strict dependency-aware structural alignment, multiple compression domains may be forced to partition in order to maintain group-level alignment across dependent domains.
% Although such partitioning preserves cross-domain alignment, it increases the total number of execution groups, thereby increasing the number of issued packed instructions.
% By selectively relaxing alignment at subgraph boundaries, each compression domain can instead be executed as a single group.
% While this may introduce additional data movement due to misaligned dependencies, the reduction in execution group count directly reduces the total number of packed instructions.
% Therefore, the construction of execution groups requires a trade-off between the data movement overhead induced by dependency alignment and the number of execution groups.


% % 在subgraph的边界考虑硬件利用效率来打破dependency-aware structural alignment
% % 如何判断是否需要 selective relaxation？
% \textit{How to determine when selective relaxation should be applied?}
% Intuitively, relaxation is beneficial only if the reduction in instruction count outweighs the additional data movement overhead it introduces.
% % 首先，我们将selective relaxation点放在subgraph的边界，而非subgraph内部。这是因为同构subgraph内部的结构和数据依赖是一致的，在 dependency-aware structural alignment 约束下，能够自然实现较高的执行单元位宽利用率。
% % 相比之下，同构subgraph的边界所连接的其他子图是无法保障同构的。此时，在 subgraph 边界处进行 selective relaxation，能够在保持子图内部结构完整性的同时，缓解严格结构对齐带来的执行组膨胀问题。
% % 其次，我们构建如下评估模型用来判断是否需要在subgraph边界执行selective relaxation。
% We apply selective relaxation at the boundaries of subgraphs rather than within them. This is because the structure and data dependencies within isomorphic subgraphs are consistent, enabling high execution unit bitwidth utilization under dependency-aware structural alignment.
% In contrast, subgraphs connected at the boundaries may not be isomorphic. In such cases, applying selective relaxation at subgraph boundaries mitigates the execution group expansion caused by strict structural alignment while preserving the internal structure of each subgraph.

% To formalize this decision, we construct an evaluation model that determines whether selective relaxation should be applied at subgraph boundaries.
% Under strict dependency-aware alignment, the total number of execution groups can be decomposed as
% \begin{equation}
% G_{\text{strict}} = G_{\text{align}} + G_{\text{res}},
% \end{equation}
% where $G_{\text{align}}$ denotes groups enforced by cross-subgraph alignment, and $G_{\text{res}}$ represents the structural lower bound imposed by intra-subgraph dependencies.

% Applying selective relaxation removes cross-subgraph alignment constraints, producing
% \begin{equation}
% C_{\text{relax}} = G_{\text{relax}} + M,
% \end{equation}
% where $G_{\text{relax}}$ is the resulting number of execution groups and $M$ is the additional data movement cost.

% The strict-alignment cost is
% \begin{equation}
% C_{\text{strict}} = G_{\text{align}} + G_{\text{res}}.
% \end{equation}

% We define the \emph{selective relaxation gain} as
% \begin{equation}
% \Phi = C_{\text{strict}} - C_{\text{relax}}.
% \end{equation}

% Selective relaxation is applied only when $\Phi > 0$, i.e., when the reduction in execution group count outweighs the introduced data movement overhead.


% Collectively，我们给出Structurally Aligned Node Grouping算法，如xxx所示。
To this end, we propose the dependency-aware dense packing algorithm, which is shown in Algorithm~\ref{alg:sang}.
% 首先，我们按照topo排序遍历compression domains。根据硬件约束，为每个compression domain提取一个最大可行execution group
% second，我们尝试根据依赖关系从后继compression domain中扩展execution group。由于compression domain保留了对同构子图中的对应节点关系。因此，我们的扩展本质上是在同构子图上做扩展
% third，我们需要判断扩展后的执行组是否合理。具体而言，首先需要满足硬件约束限制；其次，对于跨同构subgraph的扩展，需要判断是否使用selective relaxation以断开扩展来提升硬件利用率。
% 最后，我们从compression domains中删除已经对其的execution groups并重复上诉步骤。
\begin{itemize}
    \item First, the compression domains are traversed in topological order. For each domain, a maximal feasible group of nodes is selected to form an initial pack that fills a machine word as fully as possible, respecting hardware width constraints.

    \item Next, each initial pack is expanded to successor domains along dataflow dependencies. Thanks to the structural alignment maintained by compression domains, the expansion is performed over corresponding nodes in isomorphic subgraphs, ensuring that data produced by upstream packs can be directly consumed by downstream packs. Once the packs are expanded, the nodes assigned to each pack are removed from their respective domains, and the procedure repeats until all nodes are assigned to packs.

    \item Finally, the algorithm performs intra-domain pack merging. Packs belonging to the same compression domain are grouped together, and multiple packs are merged whenever the combined bit-width does not exceed the machine word size. This merging further increases bit-space utilization without introducing data reorganization overhead.

\end{itemize}

% 1. 按照topo排序，取出一个compression domain
% 2. 从compression domain中取出一个execution group，以最大化利用hardware width
% 3. 扩展execution group
% 4. hardware是否能够next execution group的合法性过滤
% 5. next execution group是否与execution group处于同一个subgraph的松弛性过滤
% 6. 继续扩展
% 7. compression domains中删除位于已扩展的execution group的节点
\begin{algorithm}[t]
\caption{Dependency-Aware Structural Alignment}
\label{alg:sang}
\begin{algorithmic}[1]
\Require Compression domains $D$, hardware width $W$
\Ensure Structurally aligned execution groups $\mathcal{E}$

% \State $\mathcal{E} \gets \emptyset$

% % \State $TopoOrder \gets$ TopologicalSort($D$) 

% \ForAll{$d \in TopologicalSort(D)$}
%     \While{$d$ contains unassigned nodes}
%         \State $g \gets$ InitializeMaxFeasibleGroup($d$, $W$) 
%             %\Comment{Maximal feasible group from domain $d$}
%         \State WorkList $\gets \{(d, g)\}$ 
%         % \Comment{Store frontier as (domain, group) tuple}

%         \While{WorkList is not empty}
%             \State Pop $(cur\_d, cur\_g)$ from WorkList
%             \State $nextDomains \gets$ SuccessorDomains($cur\_d$)

%             \ForAll{$d' \in nextDomains$}
%                 % \State $g' \gets$ ExtractDependentNodes($d'$, $g$) \Comment{Dependency-aware structural alignmen}
                    
%                 \If{CanExpand($g, g', W$)}
%                     \State $g \gets g \cup g'$ 
                    
%                     \State Remove nodes of $g'$ from $d'$ 
                    
%                     \State Push $(d', g')$ into WorkList
%                 \EndIf
%             \EndFor
%         \EndWhile

%         \State Remove nodes of $g$ from $d$
%         \State $\mathcal{E} \gets \mathcal{E} \cup \{g\}$
%     \EndWhile
% \EndFor



\State $\mathcal{E} \gets \emptyset$
\State \textcolor{blue}{// Alignment-aware packing}
\ForAll{$d \in TopologicalSort(D)$} 
    \While{$d$ contains unassigned nodes}
        % 初始化最大可行组（Max Feasible Group）
        \State $g \gets$ InitializeMaxFeasibleGroup($d$, $W$) 
        \State WorkList $\gets \{(d, g)\}$

        % 依赖感知扩展pack
        \While{WorkList is not empty}
            \State Pop $(cur\_d, cur\_g)$ from WorkList
            \State $nextDomains \gets$ SuccessorDomains($cur\_d$)

            \ForAll{$d' \in nextDomains$}
                \State $g' \gets$ ExtractDependentNodes($d'$, $cur\_g$) 
                \State $cur\_g \gets cur\_g \cup g'$ 
                \State Remove nodes of $g'$ from $d'$ 
                \State Push $(d', g')$ into WorkList
            \EndFor
        \EndWhile

        \State Remove nodes of $g$ from $d$
        \State $\mathcal{E} \gets \mathcal{E} \cup \{g\}$
    \EndWhile
\EndFor

\State \textcolor{blue}{// Pack merging}
% 域内pack合并（Intra-domain merging）
% \State $\mathcal{E}_d \gets$ PacksInDomain($d$, $\mathcal{E}$)
% \ForAll{$(g_i, g_j) \in \mathcal{E}_d$}
%     \If{CanMerge($g_i, g_j, W$)}
%         \State $g_{ij} \gets g_i \cup g_j$
%         \State Remove $g_i, g_j$ from $\mathcal{E}$
%         \State $\mathcal{E} \gets \mathcal{E} \cup \{g_{ij}\}$
%     \EndIf
% \EndFor

% 域内pack合并（按pack所属域分组）
\State Group packs in $\mathcal{E}$ by their compression domain
\ForAll{each group of packs in the same domain}
    \ForAll{pairs $(g_i, g_j)$ in the group}
        \If{CanMerge($g_i, g_j, W$)}
            \State merge $g_i$ and $g_j$ into $g_{ij}$
            \State remove $g_i, g_j$ from $\mathcal{E}$
            \State add $g_{ij}$ to $\mathcal{E}$
        \EndIf
    \EndFor
\EndFor


\State \Return $\mathcal{E}$
\end{algorithmic}
\end{algorithm}


% \subsubsection{Benefit Evaluation}
% 过滤掉没有收益的pack


==> Section/challenge3_method_v1.tex <==

\subsection{Compressed Execution Implementation}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figure/BMI3.pdf}
    \caption{
            Examples of (a) \texttt{PEXT}, (b) \texttt{PDEP}, and (d) lookup table-based compression for an (c) Eq operations group.
    }
    \label{fig:BMI}
\end{figure}


% \subsubsection{\textbf{Packed Execution Model}}

% Let $W$ denote the machine word width. We divide the word into $k$ fixed-width lanes, each occupying $b$ bits:

% \begin{equation}
% W = k \cdot b .
% \end{equation}

% Each lane corresponds to one node instance from an isomorphic subgraph. Given node values
% $\{x_0, x_1, \dots, x_{k-1}\}$, we construct a packed operand

% \begin{equation}
% X = \sum_{i=0}^{k-1} (x_i \ll (i \cdot b)).
% \end{equation}

% Another packed operand $Y$ is constructed from $\{y_0, y_1, \dots, y_{k-1}\}$, similarly.

% Executing an ALU operation $OP$ over packed operands produces

% \begin{equation}\label{op_model}
% Z = OP(X, Y).
% \end{equation}

% For correctness, the packed execution must satisfy the \emph{lane independence property}
% % : each bit or lane can be computed independently without introducing carry propagation or inter-bit dependencies

% \begin{equation}
% z_i = OP(x_i, y_i), \quad \forall i \in [0, k-1],
% \end{equation}

% where $z_i$ is the value stored in the $i$-th lane of $Z$.

\subsubsection{\textbf{Bit Manipulation Instructions}}
% 在描述special operation前，我们先介绍BMI中的两个关键指令：PEXT和PDEP，which 允许我们高效地实现bit操作。
% Shift Operation：使用PDEP实现
% Bits Operation：使用PEXT实现
% == 运算：使用PEXT+AND实现
Before describing the implementation of various operations, we first introduce two key instructions from the Bit Manipulation Instructions~(BMI) set: \texttt{PEXT} and \texttt{PDEP}. Both instructions perform bit-level manipulation based on a given mask:
\begin{itemize}
    \item \texttt{PEXT} (Parallel Bit Extract) extracts bits from a source word according to a mask and packs them contiguously into the least significant bits of the destination word. 
    % This allows selective compression of relevant bits while ignoring the rest.
    \item \texttt{PDEP} (Parallel Bit Deposit) deposits bits from a source word into a destination word according to a mask, leaving other positions unchanged. 
    % This facilitates flexible placement of bits in arbitrary positions without explicit shifts or loops.
\end{itemize}
Figure~\selfref{fig:BMI} illustrates an example of how \texttt{PEXT} and \texttt{PDEP} operate with a given mask.

\subsubsection{\textbf{Bit-level Compression for Logic Operation}}
% Logical operations (e.g., AND, OR, XOR) naturally satisfy the lane independence property because they do not introduce carry propagation across bits. Therefore, packed logical operations can be executed directly with equation \selfref{op_model}.
Logical operations, such as \texttt{AND}, \texttt{OR}, \texttt{NOT}, and \texttt{XOR}, form the majority of operations~(over 55\% shown in Figure~\selfref{fig:motivation1}~(b)) in RTL simulation.
These operations are particularly amenable to bit-level packing because they inherently satisfy the lane independence property. 
As a result, multiple lanes can be packed into a machine word and processed in parallel without additional special handling. 
Consequently, bit-level Compression for logical operations provides a straightforward and highly efficient path for accelerating RTL simulation.



\subsubsection{\textbf{Bit-level Compression for Eq operation}}
% Eq 运算在不同架构下具有不同的压缩机会。
Eq operations exhibit different compression opportunities across architectures.
% 在 AI 加速器中，由于采用了量化技术，操作数的位宽通常较低。在这种情况下，可以直接应用位级压缩方法，利用低位宽减少存储和计算开销。
In AI accelerators, due to the use of quantization techniques~\selfcite{quantization_acc1,quantization_acc2,quantization_acc3,quantization_acc4}, operands typically have low bit-widths.
Therefore, Eq operations can be implemented using \texttt{PEXT} and bitwise \texttt{AND}. 
Let $M_i$ denote the mask that selects the $i$-th bit from all lanes. 
We first extract these bits using
$
B_i = \texttt{PEXT}(X, M_i),
$
where $B_i$ contains the $i$-th bit of every lane packed contiguously. 
We then obtain the results using
$
R = \bigwedge_{i=0}^{k-1} B_i.
$
% 如果operands的位宽一样，当n小于等于5时才有收益。
Note that when operands have the same bit-width, this approach provides benefits only if the bit-width of the operands $\leq 5$.

% 而在 CPU 设计中，操作数的位宽通常为 32 位或更高，这使得低位宽压缩方法并不适用。
In contrast, for CPU designs, the bit-width of operands are typically wider, making the above methods inapplicable.
% 然而，我们发现 Eq 运算存在另一类可利用的模式：超过 95\% 的 Eq 运算属于一种Eq运算组模式，其中一组 Eq 运算共享相同的输入，而另一个输入为常量。
% 针对这一模式，我们采用查找表（lookup table）压缩方案,其中每个条目代表不同常量，Eq运算组的非常量输入作为查找表的索引。 因此，Eq运算组的计算转换成如下运算：首先使用非常量输入的上一个cycle的值作为索引对查找表中的值复位，然后使用当前cycle的值作为索引对查找表中的值置位。另外，可以使用PEXT实现并行提取。
However, we observe another exploitable pattern in Eq operations: over 95\% of Eq operations form groups in which one operand is shared among multiple operations while the other operand is a constant. 
For this pattern, we employ a lookup table-based compression scheme. Each entry in the table corresponds to a different constant, while the non-constant operand of the Eq group serves as the table index. 
As a result, the computation of the Eq group can be transformed as follows: first, the value from the previous cycle of the non-constant operand is used to reset the corresponding table entries; then, the current cycle value of the non-constant operand is used to set the table entries accordingly. 
Furthermore, \texttt{PEXT} can be leveraged to extract bits in parallel.





\subsubsection{\textbf{Bit-level Compression for Special Operation}}
% 这里，我们实现两类运算：Shift Operations 和 Bits Extraction，which 
\textbf{Shift Operations:} 
Shift-based operations, such as such as bit-width extension, can be efficiently implemented using \texttt{PDEP}.
% 在RTL simulating中，这些运算有个特点，它们存在一个常量operand。
% 因此，在编译阶段，我们可以根据其所处的lane和常量operand构建mask，然后\texttt{PDEP} deposits the source bits to their target positions at runtime.
In RTL simulation, these operations typically involve a constant operand. Therefore, at compile time we construct a mask according to the lane layout and the constant operand, and \texttt{PDEP} deposits the source bits into their target positions at runtime.
% Figure xxx~(a) 可以看成使用\texttt{PDEP}实现对xi的位宽由2扩展成4.
Figure~\selfref{fig:BMI}~(a) illustrates an example where \texttt{PDEP} is used to expand the bit-width of $x_i$ from 2 bits to 4 bits.

\textbf{Bits Extraction:} 
% 这类运算的功能是从$x_i$中提取部分bits。这类运算通常也存在一个常量输入，所以，可以使用\texttt{PEXT}来实现。类似的，我们可以在编译时构建好mask，然后运行时通过\texttt{PEXT}提取。
% Figure xxx(b)可以看出从$x_0, x_1, x_2, x_3$ 中分别提取1，2，3，3位置上bit。 
These operations extract selected bits from $x_i$. Since the extraction positions are usually specified by a constant operand in RTL simulation, we implement them using \texttt{PEXT}. A mask is generated at compile time, and \texttt{PEXT} extracts the required bits at runtime.
Figure~\selfref{fig:BMI}~(b) shows an example where bits at positions 1, 2, 3, and 3 are extracted from $x_0$, $x_1$, $x_2$, and $x_3$, respectively.

% % == 运算：使用PEXT+AND实现。具体而言，先使用PEXT提取单个位置，然后所有位置AND。
% \textbf{Equality Comparison:}
% Equality operations can be implemented using \texttt{PEXT} and bitwise \texttt{AND}. 
% Let $M_i$ denote the mask that selects the $i$-th bit from all lanes. 
% We first extract these bits using
% \[
% B_i = \texttt{PEXT}(X, M_i),
% \]
% where $B_i$ contains the $i$-th bit of every lane packed contiguously. 
% We then obtain the results using
% \[
% R = \bigwedge_{i=0}^{k-1} B_i
% \]


% 至于其他运算，由于占比很低，我们不做压缩处理。
% As for other operations, since their occurrence is rare, we do not apply any compression to them.


% \subsubsection{\textbf{Data Layout}}
% 在 RTL 仿真中，寄存器通常被建模为全局变量。为了避免数据在内存中的分布较为分散，引入额外的数据重排（data reorganization）开销，我们采用基于 pack 的数据布局（pack-based data layout）。
% 



==> Section/discussion.tex <==

\section{Discussion}
The proposed node compression optimization mitigates the CPU front-end bottleneck suffered by RTL simulation, which is orthogonal to existing methods~\selfcite{GSIM, essent, dedup, zhou2023khronos,repcut,parendi} and can be seamlessly integrated to maximize the performance of RTL simulation.

% node compression和SIMD都是data-level并行。但是它们也存在一些差异：首先，SIMD利用的是粗粒度的lane来执行数据并行而node compression利用的是细粒度的bit。其次，SIMD利用的是向量单元而node compression利用的是标量单元 that 硬件执行效率要高于向量单元。最后，本质上看来，node compression 能够减少运算量，多个节点的运算一次打包计算，而SIMD没有实现运算量的减少。
% 注意，尽管存在这些差异，但是node compressin与SIMD不冲突，可以先使用node compression来提高bit空间利用率，然后在使用SIMD近一步加速。
\textbf{Comparison with SIMD:}
Node compression and SIMD both exploit data-level parallelism but differ in granularity and efficiency: SIMD uses coarse-grained lanes on vector units, while node compression operates at fine-grained bit-level parallelism on scalar units, achieving higher hardware efficiency~\selfcite{agner_instruction_tables} and reducing computation by computing multiple nodes at once. 
Although that, both are complementary: node compression can first improve bit utilization, after which SIMD can further accelerate execution.
Future work will investigate strategies for integrating both methods.

% \textbf{Waveform friendly:}
% The proposed node compression method is well-suited for waveform dumping tasks such as debugging and power analysis~\selfcite{grannite, apollo}, offering two major benefits: faster dumping speed and smaller waveform file size.
% Waveform dumping incurs frequent and costly writes as signal values change~\selfcite{dump_slow}, but node compression enables packing multiple signals into a single machine word, reducing write overhead.
% Furthermore, waveform files often grow to tens or even hundreds of gigabytes~\selfcite{apollo}, where byte-aligned storage~\selfcite{verilator, essent} leads to severe space waste. Our method inherently avoids this limitation, reducing file size.
% Node compression in waveform dumping will be a focus of our future work.


\textbf{Limitation:} Bit-level compression execution currently applies to the operations described in Section~\selfref{sec:compression_execution}, which account for the majority of operations, while other operations are not yet supported. 

==> Section/motivation.tex <==
\section{Motivation}

\subsection{Observation}
{We perform a systematic analysis of RTL simulation task characteristics and hardware resource utilization efficiency, yielding the following key observations:}

%%%%% bit-space inefficiency 
% 我们统计了各类运算的位宽分布，如图xxx所实施，可以看到超过70%的运算的位宽都不足10bit，而现代CPU通常支持64位宽的并行运算。
% 如果像已有的工作xxx，简单地extending low bitwidth data to a standard bitwidth, such as 16-bit or 32-bit, to leverage existing hardware support for operations。It results in significant underutilization of the computational unit’s binary space, leading to inefficient resource usage, denoted as bit-space inefficiency. 
\underline{\textbf{Observation 1: Bit-space inefficiency.}} 
We analysis of the bit-width distribution of various nodes, as shown in Figure \selfref{motivation_data}~(a), reveals that over 80\% of nodes operate on less than 10 bits. 
In contrast, modern CPUs are designed to handle 64-bit operations efficiently.
Prior approaches extend these low-bitwidth operands to standard widths (e.g., 16 or 32 bits), resulting in severe underutilization of the available bit-space and inefficient use of computational resources, which we term \textit{bit-space inefficiency}.

%%%%%% RTL simulation是否为scalar computatoin-bound ？
\underline{\textbf{Observation 2: Unused Vector Execution Resources.}} 
% 


%%%%%% abundant parallelism isomorphic node （RTL graph体现出高度data-parallelsim）
\underline{\textbf{Observation 3: Abundant data-level parallelism.}} 
% 我们统计了RTL仿真中不同节点类型的占比，如图xxx所示，其中访存节点（主要是寄存器）、逻辑运算节点和算术运算节点分别占比约为xx%，xx%，xx%。可以看到，RTL仿真中存在大量的同构节点。
We quantify the distribution of node types in RTL graph, as shown in Fig.~xxx, which reveals that RTL simulation consists of a large number of isomorphic nodes that share identical operation types but differ only in operands.
% 另外，我们进一步分析了RTL graph的topological结构。如何xxx所示，the RTL graph exhibits a cone-shaped structure，with 前xxx level包含了xxx%的节点。由于相同level的节点之间不存在任何依赖关系，因此同一level的节点可以并行计算。
We further analyze the topological structure of the RTL graph. 
As shown in Fig.~xxx, the RTL graph exhibits a cone-shaped topology, where the first xxx levels already cover xxx of all nodes. Critically, nodes within the same topological level have no inter-dependencies and can therefore be computed independently.
% 因此，通过上述分析可以发现，RTL graph具备高度同构节点的数据并行。
Taken together, these results show that RTL simulation inherently contains abundant data-level parallelism: large groups of isomorphic nodes can be evaluated using the same operation, and many such nodes can be processed concurrently due to dependency-free topological organization.

% 基于以上所有observation, our method is node compression. 具体而言xxxx
Based on the above observations, we introduce \textit{node compression}, a fundamentally different execution model that shifts from node-wise execution to compressed multi-node execution. 
Instead of translating each RTL node into separate instructions, node compression aggregates a large number of isomorphic nodes and evaluates them collectively using a single instruction via bit-level parallelism and SIMD. 
This approach dramatically reduces the instruction working set and mitigates the front-end bottleneck caused by excessive instruction supply pressure.

\subsection{Challenge}
% node compression的关键挑战在于如何减少Pack&Unpack开销。
% 具体而言，什么是pack开销，什么是unpack开销。
% 尽管同一level的任何同构node都能够，但是不友好的分组会导致超出收益的pack&unpack开销，如xxx。
% 找出一个最优的方案已被证明是一个NP-hard问题，目前的启发式策略的方法是packed data produced as a result of one computation can be used directly as source in another computation，从而避免pack&unpack开销。
% 压缩不仅要看 node type，还要看 dataflow continuity
% 缺乏更大范围的子图级视野

% node compression 的核心挑战在于 pack/unpack 开销可能抵消其收益。虽然同构节点理论上可以压缩执行，但不合理的分组会导致频繁的数据重组，使 packed 数据无法在 producer-consumer 之间直接复用，从而产生额外开销。然而，寻找最优分组以最小化 pack/unpack 开销属于 NP-hard 问题。现有启发式搜索方法，依赖于use-def 或 def-use，缺乏子图级全局视角，虽然能够保证局部相邻的dataflow continuity，但是无法保证producer–consumer 跨多级 dataflow 的连续 packed execution。如图xxx所示。
Node compression faces a fundamental challenge in that the overhead of pack and unpack operations may offset its performance benefits. 
Although isomorphic nodes within the same topological level can theoretically be executed in compressed form, suboptimal grouping can introduce frequent data reorganization, preventing packed data from being directly reused between producer–consumer pairs and incurring additional overhead. 
However, finding the optimal grouping that minimizes pack/unpack overhead is an NP-hard problem~\selfcite{goSLP}. 
Existing heuristic approaches rely on \textit{use}-\textit{def} or \textit{def}-\textit{use} chains and lack a global subgraph-level perspective. 
While they preserve local dataflow continuity between adjacent nodes, they cannot guarantee globally optimal packed data reuse or minimize pack/unpack overhead across the entire computation graph.

\subsection{Opportunity}
% RTL graph 具有 module-induced structural regularity，而不是 random graph。

% RTL graph 并不是一个随机生成的图结构，而是由硬件架构通过模块实例化系统性生成的结构化图。
% 现代designs都会被设计成高并行架构，例如多个 cores、tiles、vector lanes 或 processing elements。
% 同时，这些designs通常通过复制计算模块来扩展并行性，而不是构建完全不同的逻辑结构。
% 因此，RTL graph 中包含大量重复子图，这些子图在node type，topology，dataflow pattern上高度一致。
RTL graphs are not arbitrary structures, but are systematically generated from hardware architectures through module duplication. 
Modern designs are highly parallel, incorporating multiple cores, tiles, vector lanes, or processing elements. To scale parallelism, these designs typically replicate computation modules rather than constructing entirely unique logic structures. As a result, RTL graphs contain a large number of repeated subgraphs that exhibit strong similarity in node types, topology, and dataflow patterns.

% module 在架构层和 RTL graph 层之间建立了天然的桥梁。从架构角度来看，module 表示一个可重复的计算单元；从 RTL graph 角度来看，每个 module instance 对应一个结构一致的子图。这种 module-induced structural regularity 使得可以在子图级别识别结构对齐的节点组，而不仅仅是孤立的同构节点。
Modules provide a critical bridge between architectural structure and RTL graph representation.
From an architectural perspective, modules represent reusable computational units. 
From an RTL graph perspective, each module instance corresponds to an isomorphic subgraph in the RTL graph.
This module-induced regularity exposes compression opportunities at the subgraph level, enabling structurally aligned grouping beyond isolated node-level similarity.

% 利用 module hierarchy 提供的结构信息，可以构建 compression-friendly 的节点分组。具体而言，对于同一 module 的多个 instance，基于其结构一致性，对齐不同 instance 中在拓扑结构中具有相同相对位置且执行相同操作的节点，并将这些节点打包为一个执行组。每个执行组对应 module 子图中的一个结构位置，包含来自不同 instance 的同构节点。由于这些执行组在数据流上保持结构对齐，一个执行组产生的 packed 数据可以被后续执行组直接消费，而无需进行 unpack 或 repack，从而实现 packed 数据在整个子图范围内的连续传播，并显著降低 packing 开销。
By leveraging module hierarchy, we construct compression-friendly node groupings based on structural alignment across module instances. 
Specifically, for replicated instances of the same module, we align nodes that perform the same operation and occupy the same relative position in the module’s dataflow graph, and pack them into a unified execution group. Each group corresponds to a specific structural position within the module subgraph and contains isomorphic nodes from different instances. This structural alignment preserves producer–consumer relationships across groups, allowing packed results to be directly forwarded between successive groups without unpacking or repacking. 
As a result, packed data can propagate seamlessly across subgraph execution, minimizing packing overhead and enabling efficient large-scale node compression.

% RTL graph 不是 random graph，而是 architecture-generated graph。
% Modern designs are rarely composed of unique singleton modules. Parallelism is frequently exploited, whether it be for multiple tiles, cores, vector lanes, etc. 
% 目前所有的设计都是高并行架构，如multiple tiles, cores, vector lanes, etc.  Modern designs are rarely composed of unique singleton modules。xxx往往是同一个module的不同实例。因此，RTL graph中包含大量repeated subgraphs。
% 架构级信息提供更子图级视野，如PE阵列。
% 为了构建架构级信息与RTL graph之间的关系，我们巧妙地引入module作为代理。
% 对于架构而言，module构建了
% 对于RTL graph而言，module的实例构成RTL graph的子图。

% module-aware minner algorithm

==> Section/motivation_v2.tex <==



\section{Motivation}


\subsection{Inefficiency of Node-Granular Execution}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figure/motivation1_4.pdf}
    \caption{
        % Distribution of (a) node bit-widths and (b) node type.
        % (c) Node distribution across topology levels in the RTL graph, where the x-axis denotes the topology level and the y-axis denotes the number of nodes per level.
        Distribution of (a) node bit-widths, (b) node types, and (c) node counts across topology levels in the RTL graph.
        For the Boom-8C design, the first 10\% of topology levels are remained for better visualization.
    }
    \label{fig:motivation1}
\end{figure}


{We perform a systematic analysis of RTL simulation task characteristics and hardware resource utilization efficiency, yielding the following key observations:}

%%%%% bit-space inefficiency 
% 我们统计了各类运算的位宽分布，如图xxx所实施，可以看到超过70%的运算的位宽都不足10bit，而现代CPU通常支持64位宽的并行运算。
% 如果像已有的工作xxx，简单地extending low bitwidth data to a standard bitwidth, such as 16-bit or 32-bit, to leverage existing hardware support for operations。It results in significant underutilization of the computational unit’s binary space, leading to inefficient resource usage, denoted as bit-space inefficiency. 
\underline{\textbf{Observation 1: Bit-space inefficiency.}} 
We analysis of the bit-width distribution of various nodes, as shown in Figure \selfref{fig:motivation1}~(a), reveals that over 80\% of nodes operate on less than 16 bits. 
In contrast, modern CPUs are designed to handle 64-bit operations efficiently.
Prior approaches extend these low-bitwidth operands to standard widths (e.g., 16 or 32 bits), resulting in severe underutilization of the available bit-space and inefficient use of computational resources, which we term \textit{bit-space inefficiency}.


%%%%%% abundant parallelism isomorphic node （RTL graph体现出高度data-parallelsim）
\underline{\textbf{Observation 2: Abundant data-level parallelism.}} 
% 1. 可并行的节点量大
% 2. 可并行的节点多样性低
% 结论：存在大量可并行的同构节点
% The RTL graph exhibits a highly skewed node-type distribution, dominated by a few node types. 我们统计了RTL仿真中不同节点类型的占比，如图xxx所示，其中访存节点（主要是建模寄存器）、逻辑运算节点和Eq运算节点分别占比约为xx%，xx%，xx%。因此，RTL仿真中存在大量的同构节点 share identical operation types but differ only in operands。
The RTL graph exhibits a highly skewed node-type distribution, dominated by a few node types. 
As shown in Figure~\selfref{fig:motivation1}~(b), memory-access nodes~(registers), logic operation nodes, and Eq operation nodes account for approximately 32.08\%, 55.14\%, and 8.54\% of all nodes in the Conv2D-$16\times16$ design, respectively.
This indicates the prevalence of isomorphic nodes that share identical operations but differ only in operands.
% 另外，RTL图呈现出明显的拓扑倾斜特性（highly skewed topology），即节点在不同拓扑层分布极不均衡。进一步的拓扑分析（如图所示）表明，前若干拓扑层包含了绝大多数节点。具体而言，节点数量超过1000的层，其节点总数占整个RTL图节点总数的96%以上。由于相同level的节点之间不存在任何依赖关系，因此同一level的节点可以并行计算。
Furthermore, the RTL graph exhibits a pronounced skewed topology, with nodes highly concentrated in a small number of topological levels. 
Topological analysis, as shown in Figure~\selfref{fig:motivation1}~(c), reveals that nodes are highly concentrated in the first few levels, with levels containing over 1,000 nodes accounting for more than 96\% of all nodes in the RTL graph.
Critically, nodes within the same topological level have no inter-dependencies and can therefore be computed independently.
% 因此，通过上述分析可以发现，RTL graph具备高度同构节点的数据并行。
Taken together, these results indicate that RTL simulation exhibits abundant data-level parallelism, with large groups of isomorphic nodes amenable to concurrent computation.
% Taken together, these results show that RTL simulation inherently contains abundant data-level parallelism: large groups of isomorphic nodes can be evaluated using the same operation, and many such nodes can be processed concurrently due to dependency-free topological organization.

% 基于以上所有observation, our method is node compression. 具体而言xxxx
Based on the above observations, we introduce \textit{node compression}, a fundamentally different execution model that shifts from node-wise execution to compressed multi-node execution. 
Instead of lowering each RTL node into a single instruction fragment, node compression aggregates a large number of isomorphic nodes and lowers them collectively using a single instruction fragment via bit-level parallelism. 
This approach not only dramatically reduces the instruction working set and mitigates the front-end bottleneck caused by excessive instruction supply pressure, but also decreases the computation workload by fusing multiple operations into a single execution.

\subsection{Challenge of Node Compression}
% 尽管同一拓扑层中的同构节点在理论上可以通过压缩方式实现共享执行，但在实际中，不友好的压缩方式会带来data rearrangement开销，使得压缩运算无利可图。高效的节点压缩仍面临多方面挑战。其根本原因在于，节点压缩不仅涉及结构等价性的识别，还涉及跨节点的数据布局优化以及压缩执行机制的协同设计。具体而言，主要存在以下三个方面的关键挑战：

Although isomorphic nodes within the same topological level can, in principle, share execution through compression, poorly designed compression strategies may incur substantial data rearrangement overhead, making compressed execution unprofitable. 
Therefore, achieving efficient node compression in practice is non-trivial, which faces three key challenges:
% This stems from the fact that node compression goes beyond structural equivalence identification, requiring coordinated optimization of cross-node data layout and execution mechanisms. 
% In particular, it introduces three key challenges:

% 挑战1:
\textbf{Challenge 1: Lack of a global subgraph-level perspective.} Existing heuristic approaches rely on local search, such as \textit{use}-\textit{def} or \textit{def}-\textit{use} chains~\selfcite{PLDI_2000_Larsen,ASPLOS_2021_Chen}, and are prone to being misled in the presence of numerous isomorphic nodes~\selfcite{ASPLOS_2012_Park}, 
due to compressible nodes are handled separately, lacking a holistic view of the subgraph for coordinated compression.
As shown in Figure~\selfref{fig:challenge}~(b), the suboptimal grouping incurs two rounds of data reorganization, resulting from forming groups \textit{G1} and \textit{G2} without accounting for \textit{G3}.
In contrast, the optimized grouping in Figure~\selfref{fig:challenge}~(c) reduces this overhead to a single round by leveraging isomorphic subgraphs.
However, identifying isomorphic subgraphs is NP-hard~\selfcite{graph_iso1,graph_iso2}. 
% 为了克服直接在RTL graph上识别同构子图的问题，我们利用RTL graph天然具备的结构同构性。具体而言，RTL graphs are not arbitrary structures, but are systematically generated from hardware architectures through module duplication.
To overcome the difficulty of performing direct isomorphism identification on RTL graphs, we exploit the structural regularity inherent in RTL designs. 
Specifically, RTL graphs are not arbitrary structures, but are systematically generated from hardware architectures through module duplication and different instances of the same module naturally exhibit structural isomorphism. 
% 相同module的不同instance天然具备同构性，因此，By leveraging module hierarchy, we 能够高效实现同构子图识别 in the RTL graph.
By leveraging the module hierarchy, we propose module-aware isomorphic subgraph identification method to efficiently identify isomorphic subgraphs in RTL graphs.

% Modern highly parallel designs~\selfcite{high_parallel_archi1,high_parallel_archi2,high_parallel_archi3} typically replicate computation modules rather than constructing entirely unique logic structures.


% 挑战2: bit-space利用率与数据复用效率的失配
% data reuse efficientcy 关注的是数据流的依赖顺序（横向约束），而bit-space利用率关注的是在同一拓扑层中可并行节点之间的组合优化（纵向约束）。这种纵横约束意味仅从单一维度考虑pack是不可行的。具体而言，单纯依赖数据流进行打包可能导致后续 pack 无法充分填满，从而限制整体位空间利用率。而过度追求bit-space利用率导致压缩后的数据无法在生产者–消费者之间直接复用，引入频繁的数据重排开销。
% We propose a two-pronged heuristic strategy that tackles both improve bit-space utilization and minimal data rearrangement. 我们的核心策略是，有限保证pack的连续性以减少数据重排开销，然后再使用合并策略逐步提高bit空间利用率。

\textbf{Challenge 2: Mismatch between bit-space utilization and data reuse efficiency.} 
Data reuse efficiency primarily concerns the dependency order of the data flow (horizontal constraints), whereas bit-space utilization focuses on the combinational optimization among parallelizable nodes within the same topological level (vertical constraints). 
These orthogonal constraints imply that packing nodes based on a single dimension is insufficient. 
Specifically, packing solely according to the data flow may leave subsequent packs underfilled, limiting overall bit-space utilization. Conversely, overly prioritizing bit-space utilization can prevent compressed data from being directly reused between producers and consumers, introducing frequent data rearrangement overhead.
To address this challenge, we propose a two-pronged heuristic strategy that simultaneously improves bit-space utilization while minimizing data rearrangement. 
The core idea is to first maintain continuity within each subgraph to reduce data reshuffling overhead, and then progressively enhance bit-space utilization through merging strategies.


% 挑战3:\textbf{挑战三：bit-level 并行执行与跨位依赖语义的不一致。}  
% 节点压缩通过bit-level打包将多个逻辑节点映射到同一数据字中，从而实现并行执行。然而，这种bit-level并行隐含了一个关键前提，即各bit之间相互独立（lane-independent）。该前提在逻辑运算（如AND、OR、XOR）中天然成立，但对于涉及跨位依赖的运算，则往往不再成立。具体而言，此类运算通常需要在多个bit之间进行归约或传播，从而破坏打包数据中的lane边界，导致不同节点之间发生语义干扰。因此，如何在保持bit-level并行性的同时，正确高效地支持非lane-independent运算，成为节点压缩执行阶段的核心挑战。
% 为了解决这一挑战，我们提出一种面向非lane-independent运算的压缩执行变换策略。具体而言，通过对运算进行位级分解与重组，充分利用bit manipulation unit（BMU）对相关bit进行规约与传播，并结合查找表（lookup table, LUT）高效实现EQ等跨位依赖运算，从而保证了在bit-level打包下的运算语义正确性和执行效率。

\textbf{Challenge 3: Incompatibility between bit-level parallel execution and cross-bit dependency semantics.}  
Node compression maps multiple nodes into a single machine word via bit-level packing to enable parallel execution. 
However, this approach relies on the key assumption that bits (lanes) are independent. 
While this assumption holds naturally for logic operations, it breaks down for operations involving cross-bit dependencies. Such operations require reduction or propagation across multiple bits, which disrupts lane boundaries and leads to semantic interference among packed nodes. 
Therefore, efficiently supporting non-lane-independent operations while preserving bit-level parallelism remains a critical challenge in compressed execution.
To address this challenge, we propose a compression-execution transformation strategy for non-lane-independent operations. 
Specifically, operations are decomposed and reorganized at the bit level, fully leveraging the bit manipulation unit (BMU) to reduce and propagate relevant bits. Cross-bit dependent operations, such as Eq operations, are efficiently implemented using lookup tables (LUTs). 
This approach ensures both semantic correctness and execution efficiency under bit-level packed execution.


\subsection{Challenge of Node Compression}
% node compression的关键挑战在于如何减少Pack&Unpack开销。
% 具体而言，什么是pack开销，什么是unpack开销。
% 尽管同一level的任何同构node都能够，但是不友好的分组会导致超出收益的pack&unpack开销，如xxx。
% 找出一个最优的方案已被证明是一个NP-hard问题，目前的启发式策略的方法是packed data produced as a result of one computation can be used directly as source in another computation，从而避免pack&unpack开销。
% 压缩不仅要看 node type，还要看 dataflow continuity
% 缺乏更大范围的子图级视野

% node compression 的核心挑战在于 pack/unpack 开销可能抵消其收益。虽然同构节点理论上可以压缩执行，但不合理的分组会导致频繁的数据重组，使 packed 数据无法在 producer-consumer 之间直接复用，从而产生额外开销。然而，寻找最优分组以最小化 pack/unpack 开销属于 NP-hard 问题。现有启发式搜索方法，依赖于use-def 或 def-use，缺乏子图级全局视角，虽然能够保证局部相邻的dataflow continuity，但是无法保证producer–consumer 跨多级 dataflow 的连续 packed execution。
Node compression faces a fundamental challenge in that the overhead of pack and unpack operations may offset its performance benefits. 
Although isomorphic nodes within the same topological level can theoretically be executed in compressed form, suboptimal grouping can introduce frequent data reorganization, preventing packed data from being directly reused between producer–consumer pairs and incurring data reorganization overhead. 
However, finding the optimal grouping that minimizes such overhead is an NP-hard problem~\selfcite{goSLP,ASPLOS_2021_Chen}. 
Existing heuristic approaches rely on local search, such as \textit{use}-\textit{def} or \textit{def}-\textit{use} chains~\selfcite{PLDI_2000_Larsen,ASPLOS_2021_Chen}, and are prone to being misled in the presence of numerous isomorphic nodes~\selfcite{ASPLOS_2012_Park}, due to their lack of a global subgraph-level perspective.
% 如图Figure xxx所示，不好的分组，as shwon in 图(b)，导致两次data reorangement ovheread 由于没有考虑节点4和5，而好的分组，as shwon in 图(c)，只需要一次data reorangement。
As shown in Figure~\selfref{fig:challenge}~(b), the suboptimal grouping incurs two rounds of data reorganization, resulting from forming groups \textit{G1} and \textit{G2} without accounting for \textit{G3}.
% , as the group of nodes 4 and 5 is not jointly considered. 
In contrast, the optimized grouping in Figure~\selfref{fig:challenge}~(c) reduces this overhead to a single round by leveraging isomorphic subgraphs.
% 不幸的是，识别同构子图又是NP-hard问题。
Unfortunately, identifying isomorphic subgraphs is NP-hard~\selfcite{graph_iso1,graph_iso2}. However, RTL graphs exhibit special structure that allows efficient extraction of isomorphic subgraphs.
% Existing heuristic approaches rely on local search, such \textit{use}-\textit{def} or \textit{def}-\textit{use} chain~\selfcite{PLDI_2000_Larsen,ASPLOS_2021_Chen}, which prone to be fooled when a large number of isomorphic nodes exists~\selfcite{ASPLOS_2012_Park} due to lack a global subgraph-level perspective. 
% While they preserve local dataflow continuity between adjacent nodes, they cannot guarantee globally optimal packed data reuse or minimize pack/unpack overhead across the entire computation graph, especially when a large number of isomorphic nodes exists~\selfcite{ASPLOS_2012_Park}.

% \TODO{Comparison with super-word level parallelism}
% 参考 SIMD Defragmenter: Efficient ILP Realization on Data-parallel Architectures，要写出与SLP的本质区别
% 1. 搜索空间大：searching potential parallelism inside the basic block 而 rtl simulation 只存在一个超大的basic block
% 2. 缺乏子图级视野：the local scope of superword level parallelism may be fooled into selecting packing instructions when a large number of isomorphic instructions exists.


\subsection{Architecture-Induced Structural Opportunity}
% RTL graph 具有 module-induced structural regularity，而不是 random graph。

% RTL graph 并不是一个随机生成的图结构，而是由硬件架构通过模块实例化系统性生成的结构化图。
% 现代designs都会被设计成高并行架构，例如多个 cores、tiles、vector lanes 或 processing elements。
% 同时，这些designs通常通过复制计算模块来扩展并行性，而不是构建完全不同的逻辑结构。
% 因此，RTL graph 中包含大量重复子图，这些子图在node type，topology，dataflow pattern上高度一致。
RTL graphs are not arbitrary structures, but are systematically generated from hardware architectures through module duplication. 
Modern designs are highly parallel, incorporating multiple cores, tiles, vector lanes, or processing elements~\selfcite{high_parallel_archi1,high_parallel_archi2,high_parallel_archi3}. 
To scale parallelism, these designs typically replicate computation modules rather than constructing entirely unique logic structures. As a result, RTL graphs contain a large number of repeated subgraphs that exhibit strong similarity in node types, topology, and dataflow patterns.

% module 在架构层和 RTL graph 层之间建立了天然的桥梁。从架构角度来看，module 表示一个可重复的计算单元；从 RTL graph 角度来看，每个 module instance 对应一个结构一致的子图。这种 module-induced structural regularity 使得可以在子图级别识别结构对齐的节点组，而不仅仅是孤立的同构节点。
Modules provide a critical bridge between architectural structure and RTL graph representation.
From an architectural perspective, modules represent reusable computational units. 
From an RTL graph perspective, each module instance corresponds to an isomorphic subgraph in the RTL graph.
This module-induced regularity exposes compression opportunities at the subgraph level, enabling structurally aligned grouping beyond isolated node-level similarity.

% 利用 module hierarchy 提供的结构信息，可以构建 compression-friendly 的节点分组。具体而言，对于同一 module 的多个 instance，基于其结构一致性，对齐不同 instance 中在拓扑结构中具有相同相对位置且执行相同操作的节点，并将这些节点打包为一个执行组。每个执行组对应 module 子图中的一个结构位置，包含来自不同 instance 的同构节点。由于这些执行组在数据流上保持结构对齐，一个执行组产生的 packed 数据可以被后续执行组直接消费，而无需进行 unpack 或 repack，从而实现 packed 数据在整个子图范围内的连续传播，并显著降低 packing 开销。
By leveraging module hierarchy, we construct compression-friendly node groupings based on structural alignment across module instances. 
Specifically, for replicated instances of the same module, we align nodes that perform the same operation and occupy the same relative position in the module’s dataflow graph, and pack them into a unified execution group. Each group corresponds to a specific structural position within the module subgraph and contains isomorphic nodes from different instances. This structural alignment preserves producer–consumer relationships across groups, allowing packed results to be directly forwarded between successive groups without unpacking or repacking. 
As a result, packed data can propagate seamlessly across subgraph execution, minimizing packing overhead and enabling efficient large-scale node compression.

% RTL graph 不是 random graph，而是 architecture-generated graph。
% Modern designs are rarely composed of unique singleton modules. Parallelism is frequently exploited, whether it be for multiple tiles, cores, vector lanes, etc. 
% 目前所有的设计都是高并行架构，如multiple tiles, cores, vector lanes, etc.  Modern designs are rarely composed of unique singleton modules。xxx往往是同一个module的不同实例。因此，RTL graph中包含大量repeated subgraphs。
% 架构级信息提供更子图级视野，如PE阵列。
% 为了构建架构级信息与RTL graph之间的关系，我们巧妙地引入module作为代理。
% 对于架构而言，module构建了
% 对于RTL graph而言，module的实例构成RTL graph的子图。

% module-aware minner algorithm

==> Section/motivation_v3.tex <==



\section{Motivation \& Challenge}


\subsection{Inefficiency of Node-Granular Execution}

\begin{figure}[htbp]
    % \setlength{\abovecaptionskip}{0.10cm}
    % \setlength{\belowcaptionskip}{0.10cm}
    \SetCaptionSpacing{0.10cm}{0.10cm}
    \centering
    \includegraphics[width=\linewidth]{Figure/motivation1_4.pdf}
    \caption{
        % Distribution of (a) node bit-widths and (b) node type.
        % (c) Node distribution across topology levels in the RTL graph, where the x-axis denotes the topology level and the y-axis denotes the number of nodes per level.
        Distribution of (a) Node bit-widths, (b) Node types, and (c) Node counts across topology levels in the RTL graph.
        For the Boom-8C design, the first 10\% of topology levels are reserved for better visualization.
    }
    \label{fig:motivation1}
\end{figure}


{We perform a systematic analysis of RTL simulation task characteristics and hardware resource utilization efficiency, yielding the following key observations:}

%%%%% bit-space inefficiency 
% 我们统计了各类运算的位宽分布，如图xxx所实施，可以看到超过70%的运算的位宽都不足10bit，而现代CPU通常支持64位宽的并行运算。
% 如果像已有的工作xxx，简单地extending low bitwidth data to a standard bitwidth, such as 16-bit or 32-bit, to leverage existing hardware support for operations。It results in significant underutilization of the computational unit’s binary space, leading to inefficient resource usage, denoted as bit-space inefficiency. 
\textbf{Observation 1: Bit-space inefficiency.}
Our analysis of the bit-width distribution of various nodes in RTL graphs, as shown in Figure \selfref{fig:motivation1}~(a), reveals that over 80\% of nodes operate on fewer than 16 bits. 
In contrast, modern CPUs are designed to handle 64-bit operations efficiently.
Prior works~\selfcite{GSIM, essent, dedup, zhou2023khronos,repcut,parendi,verilator} extend these low-bitwidth operands to standard widths (e.g., 16 or 32 bits), resulting in severe under-utilization of the available bit-space and inefficient use of computational resources, which we term \textit{bit-space inefficiency}.
% 在xxx可以看到，在有些设计中，bit利用率不足20%。
We evaluate a set of benchmarks, as detailed in Section~\selfref{sec:bit_utilization}, and observe that certain designs exhibit critically low bit-space utilization, with utilization below 20\%.

%%%%%% abundant parallelism isomorphic node （RTL graph体现出高度data-parallelsim）
\textbf{Observation 2: Abundant data-level parallelism.}
% 1. 可并行的节点量大
% 2. 可并行的节点多样性低
% 结论：存在大量可并行的同构节点
% The RTL graph exhibits a highly skewed node-type distribution, dominated by a few node types. 我们统计了RTL仿真中不同节点类型的占比，如图xxx所示，其中访存节点（主要是建模寄存器）、逻辑运算节点和Eq运算节点分别占比约为xx%，xx%，xx%。因此，RTL仿真中存在大量的同构节点 share identical operation types but differ only in operands。
The RTL graph exhibits a highly skewed node-type distribution, dominated by a few node types. 
As shown in Figure~\selfref{fig:motivation1}~(b), memory-access nodes~(e.g., registers declared in RTL designs), logic operation nodes, and Eq operation nodes account for approximately 32.08\%, 55.14\%, and 8.54\% of all nodes in the Conv2D-$16\times16$ design, respectively.
This indicates the prevalence of \textit{isomorphic nodes} that share the identical operation type but differ only in operands.
% 另外，RTL图呈现出明显的拓扑倾斜特性（highly skewed topology），即节点在不同拓扑层分布极不均衡。进一步的拓扑分析（如图所示）表明，前若干拓扑层包含了绝大多数节点。具体而言，节点数量超过1000的层，其节点总数占整个RTL图节点总数的96%以上。由于相同level的节点之间不存在任何依赖关系，因此同一level的节点可以并行计算。
Furthermore, the RTL graph also exhibits a pronounced skewed topology, with nodes highly concentrated in a small number of topological levels. 
Topological analysis, as shown in Figure~\selfref{fig:motivation1}~(c), reveals that nodes are highly concentrated in the first few levels, with levels containing over 1,000 nodes accounting for more than 96\% of all nodes in the RTL graph.
Critically, nodes within the same topological level have no inter-dependencies and can therefore be computed independently.
% 因此，通过上述分析可以发现，RTL graph具备高度同构节点的数据并行。
Taken together, these characteristics exhibited by RTL graphs indicate that RTL simulation exhibits abundant data-level parallelism, with large groups of isomorphic nodes amenable to concurrent computation.
% Taken together, these results show that RTL simulation inherently contains abundant data-level parallelism: large groups of isomorphic nodes can be evaluated using the same operation, and many such nodes can be processed concurrently due to dependency-free topological organization.

% 基于以上所有observation, our method is node compression. 具体而言xxxx
Based on the above observations, we propose \textit{node compression} implemented via bit-level data parallelism, a fundamentally different execution model that shifts from node-wise execution to compressed multi-node execution. 
% Instead of lowering each RTL node into a single instruction fragment, node compression aggregates a large number of isomorphic nodes and lowers them collectively using a single instruction fragment via bit-level parallelism. 
Instead of lowering each RTL node into an individual instruction sequence, node compression aggregates a large number of parallelizable isomorphic nodes and lowers them collectively into a single instruction sequence via bit-level parallelism.
This approach not only dramatically reduces the instruction working set and mitigates the front-end bottleneck caused by instruction cache misses, but also decreases the computation workload by fusing multiple nodes into a single execution.



\input{Section/challenge_revision}

% \input{Section/challenge}

==> Section/overview.tex <==

\begin{figure}[htbp]
    % \setlength{\abovecaptionskip}{0.10cm}
    % \setlength{\belowcaptionskip}{0.10cm}
    \SetCaptionSpacing{0.10cm}{0.10cm}
    \centering
    \includegraphics[width=0.97\linewidth]{Figure/framework8.pdf}
    \caption{
        An overview of \papertitle{}.
    }
    \label{fig:framework}
\end{figure}




\subsection{Overview}
% As illustrated in Figure~\selfref{fig:framework}, the \papertitle{} framework takes FIRRTL~\selfcite{firrtl_sepc} code~(Flexible Intermediate Representation for RTL) as input and finally emits a C++ file, which can be compiled to generate a compiled cycle-based RTL simulator. 
As illustrated in Figure~\selfref{fig:framework}, the \papertitle{} framework takes FIRRTL~\selfcite{firrtl_sepc} files (Flexible Intermediate Representation for RTL) as input, applies bit-level data parallelism to compress nodes in the RTL graph, and ultimately lowers it to a C++ file that can be compiled into a cycle-based RTL simulator.

To address those challenges in node compression, the framework introduces the following methods.
To overcome challenge 1, we propose a module-aware isomorphic subgraph identification method~(Section~\selfref{sec:subgraph_identification}) that leverages the inherent isomorphism across module instances to reduce the search complexity.
% , providing a sub-level compression perspective.
To overcome challenge 2, we introduce an alignment-aware dense packing heuristic method~(Section~\selfref{sec:packing}) that prioritizes data reuse while improving bit-space efficiency.
% ,  achieving a trade-off between these two objectives.
To overcome challenge 3, we exploit the distinct patterns exhibited by cross-\subwordTerm{} dependent operations, and use bit manipulation instructions and lookup tables to enable bit-level parallel execution~(Section~\selfref{sec:compression_execution}).
% 为了克服挑战1，我们提出了module-aware isomorphic subgraph identification方法，该方法利用module不同实例之间的天然同构性，巧妙地避免了使用naive的同构子图挖掘算法 that is 指数级时间复杂度。
% 为了克服挑战2，我们提出了dependency-aware dense packing方法，该方法遵循data reuse优先，bit-space利用率其次的启发式策略，有效地缓解了data reuse与bit-space利用率之间的冲突。
% 为了克服挑战3，我们根据不同non-lane-independent运算表现出的不同pattern特性，提出使用bit manipulation instruciton set和look-up table来实现bit-level parallel 执行。



==> Section/performance_perf_v1.tex <==


\subsubsection{\textbf{Perf event comparison}}

%%%%% 这个版本要 IPC + instruction 
\subsubsection{\textbf{Perf event comparison}}
\begin{figure}
    \setlength{\abovecaptionskip}{0.10cm}
    \setlength{\belowcaptionskip}{0.10cm}
    \centering
    \includegraphics[width=1\linewidth]{Figure/perf3.pdf}
    \caption{
    L1I MPI~(a) and Memoey Access PKI~(b) of all simulators.
    }
    \label{fig:perf}
\end{figure}
% perf event 对比 
To further analyze the performance gap among simulators, we collected hardware performance counters using Perf~\selfcite{perf}, a powerful CPU performance analysis tool for Linux. The results are summarized in Table~\selfref{plat1_perf_cmp}.
On average, \papertitle{} achieves the highest instruction per clock (IPC)~(2.09), indicating more efficient utilization of CPU execution resources. 
In terms of the executed instruction count, \papertitle{} also executes fewer instructions than the other simulators, with the exception of Verilator. 
This demonstrates that \papertitle{} not only reduces the number of executed instructions but also executes them more efficiently, thereby delivering the best overall performance.

Although Verilator executes fewer instructions than \papertitle{}, its execution suffers from frequent instruction cache misses. 
% As shown in Figure~\selfref{l1i_mpki} 展示了Verilator和\papertitle{}的L1i MPKI数据，可以看到，Verilator几乎是\papertitle{}的一倍, 频繁的指令cache miss容易影响CPU front-end的指令供应，最后导致CPU无法满状态工作. 
% As shown in Figure~\selfref{fig:perf}~(a), Verilator experiences nearly twice the number of L1 instruction cache misses per kilo instructions~(L1i MPKI) compared to \papertitle{}. 
As shown in Figure~\selfref{fig:perf}~(a), Verilator exhibits 1.56$\times$ higher L1 instruction cache misses per kilo instructions~(L1i MPKI) on average compared to \papertitle{}, and up to 1.90$\times$ in the worst case.
Such frequent instruction cache misses limit the CPU front end’s ability to supply instructions, preventing the pipeline from achieving full utilization. 
Consequently, Verilator’s overall performance remains inferior to~\papertitle{}.

% 相比之下，Dedup 在 Rocket-8C 和 Boom-8C 设计下的 L1i MPKI 低于 ~\papertitle{}。然而，Dedup 采用code reuse的方式来减少code footpr，这会在仿真过程中引入额外的间接内存访问。如图 XX 所示，平均而言，Dedup 每千条指令的内存访问次数是 ~\papertitle{} 的 1.71 倍，最高达到 1.94 倍。这部分额外的内存开销抵消了 L1i MPKI 降低带来的优势，导致 Dedup 的整体仿真性能仍低于 ~\papertitle{}。
% In contrast, Dedup exhibits lower L1i MPKI than ~\papertitle{} for the Rocket-8C and Boom-8C designs. However, Dedup employs code reuse to reduce the code footprint, which introduces indirect memory accesses during simulation. 
Dedup, on the other hand, exhibits lower L1i MPKI than ~\papertitle{} for the Rocket-8C and Boom-8C designs. However, Dedup employs code reuse to reduce the code footprint, which introduces indirect memory accesses during simulation~\selfcite{dedup}.
% ARMOR不仅不存在indirect memory access，还能够压缩访存节点，也能过减少访存。
In contrast, ~\papertitle{} not only avoids such overhead by unfolding the RTL graph but also compresses memory access nodes shown in Figure~~\selfref{fig:compression_rate} reducing memory accesses.
As shown in Figure~\selfref{fig:perf}~(b), on average, Dedup performs 1.71 $\times$ more memory accesses per kilo instructions than ~\papertitle{}, reaching a maximum of 1.94 $\times$. This memory overhead offsets the benefit of reduced L1i MPKI, resulting in overall simulation performance that remains inferior to ~\papertitle{}.



\begin{table*}[h]
\centering
\setlength{\abovecaptionskip}{0.10cm}
\setlength{\belowcaptionskip}{0.10cm}
\caption{IPC and instruction count comparison of various simulators.}
\label{plat1_perf_cmp}
\resizebox{\textwidth}{!}{
\begin{tabular}{
        % l|r|r|r|r|r|r|r|r|r|r|r|r
        l|
        r|r|r|r|r|>{\columncolor{gray!10}}r| % 第6列灰色
        r|r|r|r|r|>{\columncolor{gray!10}}r  % 第12列灰色
    } 
\hline
\multirow{2}{*}{\textbf{Benchmark}} & \multicolumn{6}{c|}{\textbf{IPC}} & \multicolumn{6}{c}{\textbf{Instruction~(B)}} \\
\cline{2-13}
 & Repcut & Khronos & Verilator & Dedup & ESSENT & ~\papertitle & Repcut & Khronos & Verilator & Dedup & ESSENT & ~\papertitle  \\
\hline
\hline
 & 1.79 & 2.3 & 2.31 & 2 & 1.52 & 2.79 & 13.92 & 13.37 & 8.75 & 32.33 & 35.29 & 8.01 \\
 & 2.07 & 1.86 & 0.96 & 1.23 & 0.95 & 2.28 & 158.69 & 162.59 & 77.24 & 432.19 & 465.36 & 74.53 \\
 & 2.2 & 2.05 & 1.63 & 2.17 & 2.3 & 2.09 & 3.96 & 3.46 & 4.34 & 9.7 & 10.01 & 2.92 \\
 & 1.85 & 2.05 & 0.81 & 2.16 & 2.15 & 2.3 & 34.27 & 25.53 & 36.1 & 94.84 & 90.68 & 23.11 \\
 & 2.5 & 2.39 & 1.87 & 1.6 & 2.29 & 2.57 & 78.74 & 99.12 & 48.45 & 46.39 & 44.1 & 62.61 \\
 & 1.75 & 1.18 & 0.88 & 1.4 & 1.54 & 2.12 & 205.71 & 256.05 & 117.54 & 132.84 & 142.59 & 177.62 \\
 & 1.46 & - & 1.03 & 1.21 & 1.18 & 2.11 & 332.56 & 0 & 159.54 & 214.83 & 238.02 & 257.31 \\
 & 1.31 & - & 0.83 & 0.86 & 0.73 & 1.58 & 1209.41 & 0 & 562.58 & 702.17 & 783.99 & 738.24 \\
\hline
Average &  &  &  &  &  &  &  & &  &  &  &  \\
\hline
\end{tabular}
}
\end{table*}

==> rebuttal/rebuttal.tex <==

\section{Rebuttal Appendix}


We sincerely thank the reviewers for their careful reading and constructive feedback. We have revised the paper to better clarify ARMOR’s motivation, distinction from SLP/vectorization, node compression and packing details, portability, and evaluation. All review-driven changes are highlighted in red in the revised manuscript. We address the questions below.

\subsection{Response to Reviewer \#54A:}

\question{
% Q1: Justify the need to preserve a fully unrolled RTL graph. Why is full unrolling necessary rather than a historical artifact of existing simulators? How does this choice compare with compiler approaches such as loop vectorization and SLP vectorization?
Q1: Why preserve fully unrolled RTL graphs? Is full unrolling necessary, or just a legacy artifact? Compare with loop/SLP vectorization.}

% A1: ARMOR does not claim that fully unrolled RTL is the only possible representation; rather, it preserves this representation because it remains the common substrate for high-performance RTL simulation. Full unrolling makes signal addresses and dataflow dependencies statically visible, enabling hard-coded accesses and aggressive compiler optimizations. Thus, full unrolling is not merely a historical artifact. Loop-based representations do exist, such as RTeAAL Sim; however, according to its evaluation, its best configuration still does not outperform ESSENT-O2, and RTeAAL Sim attributes ESSENT-O2’s advantage to straight-line code aggressively optimized by the compiler. Compared with loop vectorization or SLP vectorization, ARMOR does not rely on loop structures or compiler-discovered vector patterns; instead, it uses RTL-specific structural isomorphism to compress nodes in an already specialized RTL graph. Therefore, ARMOR addresses the main drawback of fully unrolled RTL—large instruction footprint—without rolling the graph back into loop-based kernels.
% A1: ARMOR does not claim that fully unrolled RTL is the only viable representation; we preserve it because it remains the common substrate for high-performance RTL simulation. Full unrolling exposes signal addresses and dataflow dependencies statically, enabling hard-coded accesses and aggressive compiler optimization, hence it is not a mere legacy artifact. Loop-based representations exist (e.g., RTeAAL Sim), yet its best configuration still underperforms ESSENT-O2, which RTeAAL Sim attributes to straight-line code being aggressively compiler-optimized. Unlike loop/SLP vectorization, ARMOR does not depend on loop structures or compiler-discovered vector patterns; it exploits RTL-specific structural isomorphism to compress nodes. Thus, ARMOR mitigates the main drawback of fully unrolled RTL—large instruction footprint—without regressing to loop-based kernels.

A1: ARMOR does not claim that fully unrolled RTL is the only viable representation; we preserve it because it remains the common substrate for high-performance RTL simulation. Full unrolling exposes signal addresses and dataflow dependencies statically, enabling hard-coded accesses and aggressive compiler optimizations, hence it is not a mere legacy artifact. Unlike loop/SLP vectorization, ARMOR does not depend on loop structures or compiler-discovered vector patterns; it exploits RTL-specific structural isomorphism to compress nodes. 
% Thus, ARMOR mitigates the main drawback of fully unrolled RTL—large instruction footprint—without regressing to a rolled representation..

\revision{
R1: We have revised the introduction to make this rationale explicit.
}

% =====
\question{
Q2: Explain node compression clearly in the introduction using a concrete example: what bits are packed, what instructions execute the pack, and what exact constraints make a set of nodes compressible?
}

A2: 
% Node compression is bit-level packed execution over scalar host machine words. By structurally aligned/isomorphic nodes, we mean nodes that correspond to the same local node in the same RTL module definition across different module instances: they have identical operation semantics, bitwidths, and local dataflow structure, while only the concrete operand instances and runtime values differ. For example, if four independent 1-bit aligned nodes compute ci = ai \& bi, ARMOR packs a0–a3 into different bit slices of one word A and b0–b3 into another word B; a single scalar bitwise instruction C = A \& B then produces c0–c3 in the corresponding bit slices. Thus, logical operations such as AND/OR/XOR/NOT are executed by ordinary scalar bitwise instructions. Memory nodes correspond to simulator state variables that hold RTL register values, and ARMOR uses a pack-aligned memory layout so that one load/store transfers the whole pack. PDEP/PEXT are only used for operations requiring bit rearrangement or cross-slice handling, such as Eq, shift, bit extraction, and data rearrangement; LUT-based execution is also used for Eq groups when applicable. A set of nodes is compressible only if the nodes are structurally aligned, have no intra-pack dependencies, belong to operations supported by ARMOR’s compressed execution schemes, and do not introduce excessive data-rearrangement overhead; otherwise ARMOR falls back to uncompressed scalar execution.
% Node compression executes structurally aligned nodes by bit-level packing over scalar host words. 
% Structurally aligned nodes are the counterpart nodes across different instances of the same RTL module: they share the same operation type, bitwidth, and local dataflow structure, while only concrete operands and runtime values differ.
% For example, for four structurally aligned 1-bit nodes computing ci = ai \& bi, ARMOR packs a0–a3 into bit slices of word A and b0–b3 into word B; one scalar bitwise instruction C = A \& B produces c0–c3 in the corresponding slices. 
% Thus, logic operations such as AND/OR/XOR/NOT use scalar bitwise instructions. 
% Memory nodes, which store RTL register states in the simulator, use a pack-aligned layout so one scalar load/store instruction transfers the whole pack. 
% PDEP/PEXT are used for bit rearrangement or cross-slice operations, such as Eq, shift, bit extraction; LUT-based execution is used for Eq groups when applicable. 
% Nodes are compressible only when they are structurally aligned, have no intra-pack dependencies, are supported by ARMOR’s compressed execution schemes, and do not cause excessive data-rearrangement overhead; otherwise ARMOR falls back to uncompressed scalar execution.
Structurally aligned nodes are counterpart nodes across instances of the same RTL module, sharing an identical operation type. ARMOR packs them into bit slices of scalar host words. For example, four aligned 1-bit nodes $c_i = a_i \mathbin{\&} b_i$ are computed by packing $a_0$--$a_3$ into $A$, $b_0$--$b_3$ into $B$, and issuing one scalar bitwise $C = A \mathbin{\&} B$. Logic operations thus map to scalar bitwise instructions. Memory nodes use a pack-aligned layout, transferring the whole pack via one scalar load/store. PDEP/PEXT handle bit rearrangement and cross-slice operations; LUT-based execution covers equality groups when applicable. Compression applies only when nodes are structurally aligned, have no dependencies that prevent parallel execution within a pack, and are supported by ARMOR's compression schemes; otherwise, ARMOR falls back to uncompressed scalar execution.

\revision{
R2: Thank you for the suggestion. We agree that node compression should be introduced clearly, but the exact packed bits, execution mechanisms, and compressibility constraints depend on the methodology. Therefore, the introduction now uses a qualitative example to convey the basic idea and front-end benefit, while the detailed packing procedure, execution schemes, and constraints are described in the method sections. In particular, we have revised Section 4.3 to explicitly state the packing constraints
}


% =====
\question{
Q3: Provide subgraph-level profiling to support the rationale: number and size of isomorphic subgraphs, packability, data rearrangement cost, and lost opportunities.
}

% 我们新增了一个motivation章节，Section 3.2，which 展示了sub-graph level的profiing，包含 同构子图的数量、平均大小以及所有同构节点占RTL graph的比例。
% 另外，我们在实验部分，Figure 10 展示了node compression的占比，data rearrangement开销及node compression的净收益。
% A3: We have added a new motivation subsection, Section 3.2, where we include subgraph-level profiling of isomorphic subgraphs, shown in Figure 5. 
% The profiling reports the number of isomorphic subgraph instances across arbitrary subgraph structures, their average size, and their coverage, defined as the percentage of RTL nodes contained in such subgraphs. 
% In addition, in the evaluation section, Figure 10 reports the fraction of node compression, the data-rearrangement overhead, and the resulting net gain.


A3: We have added a new motivation subsection, Section 3.2, where we include subgraph-level profiling of isomorphic subgraphs, shown in Figure 5. In addition, in the evaluation section, Figure 10 reports the fraction of node compression, the data-rearrangement overhead, and the resulting net gain.

% =====
% \question{
% Q4: Rewrite Section 4.2 and Algorithm 1 with a step-by-step example. Clarify why the proposed module-aware identification avoids the general subgraph-isomorphism problem and what cases it intentionally does not handle.
% }

\question{
Q4: Clarify why the proposed module-aware identification avoids the general subgraph-isomorphism problem and what cases it intentionally does not handle.
}

% A4: ARMOR avoids the general subgraph-isomorphism problem because it does not mine arbitrary unknown isomorphic subgraphs from the whole RTL graph. Instead, it leverages high-level prior knowledge from the RTL design hierarchy: instances of the same module are generated from the same RTL definition, so their internal nodes have a deterministic structural correspondence after elaboration. ARMOR therefore identifies candidate isomorphic subgraphs by module type and aligns corresponding nodes using intra-module node identity. This reduces the problem from general graph matching to deterministic grouping across module instances. By design, ARMOR does not rely on discovering additional isomorphism opportunities within a module or between different module definitions; exploiting such opportunities would require more general isomorphic-subgraph mining and is beyond the scope of the current module-aware approach.


A4: ARMOR avoids the general subgraph-isomorphism problem by leveraging high-level prior knowledge: instances of the same module are generated from the same RTL definition, so their internal nodes have a deterministic structural correspondence after elaboration.
Therefore, ARMOR identifies candidate isomorphic subgraphs by module type and aligns nodes using intra-module node identity, reducing graph matching to deterministic grouping across module instances. By design, ARMOR does not discover isomorphism opportunities within a module or between different module definitions, which would require more general isomorphic-subgraph mining.



% =====
\question{
Q5: Clarify the compilation pipeline from RTL/FIRRTL to generated C++ and target ISA instructions. How exactly are PDEP and PEXT emitted and used?
}

A5: ARMOR performs node compression before C++ code generation. Starting from FIRRTL, ARMOR identifies isomorphic subgraphs, packs structurally aligned nodes into machine-word-sized packs, and then lowers each pack into an operation-specific C++ implementation. During code generation, slice-independent operations are emitted as scalar bitwise operations; for cross-slice or layout-manipulation operations that require bit deposition/extraction, ARMOR explicitly emits BMI2 intrinsics such as \_pext\_u64 and \_pdep\_u64. These intrinsics are then lowered by the compiler to target PEXT/PDEP instructions on BMI2-supported platforms.
% ARMOR does not rely on compiler-recognized C++ idioms, inline assembly, or later LLVM pattern matching to generate these instructions.

\revision{
R5: We have revised the overview in Section 4.1 and Figure 7 to clarify the full pipeline from FIRRTL to generated C++. 
% We have also added a “Portability of BMI2” discussion in Section 6.
}

% =====
\question{
Q6: Strengthen benchmark selection with manually designed accelerators such as Gemmini and FEATHER, and larger CPU configurations such as MegaBoom.
}

A6: We have strengthened the benchmark by adding Gemmini-32$\times$32 and MegaBoom-8C. The updated performance comparison is shown in Figure 9. On these new benchmarks, ARMOR still achieves the best performance among the evaluated simulators.
% , with especially strong improvement on Gemmini-32$\times$32 due to its highly regular replicated structure.

% =====
\question{
Q7: Add ablations isolating each heuristic: module-aware subgraph identification, alignment-aware packing, greedy merging, and operation-specific compressed execution.
}

% A7: We have added a ablation study to estimate the contribution of each component in ARMOR. The results show that the full ARMOR design achieves the best performance across the evaluated designs, confirming that module-aware identification, alignment-aware packing, greedy merging, and operation-specific compressed execution each contribute to profitable node compression. In particular, module-aware identification has the largest overall impact because it provides a subgraph-level view for pack discovery, while operation-specific execution is especially important for designs with many cross-slice operations. Please see Section 5.8 (\textit{Ablation Study}) and Figure \selfref{fig:ablation} for the detailed setup and results.

A7: We have added an ablation study in Section 5.8.2, in which each ARMOR component is removed individually to quantify its contribution. As shown in Figure 19 (c), the full ARMOR design achieves the best performance, confirming that each component contributes to profitable node compression.

% \revision{
% R7: We have added Section 5.8 (\textit{Ablation Study}) and Figure \selfref{fig:ablation}, which define and evaluate the variants \textit{w/o Module-aware}, \textit{w/o Align-aware}, \textit{w/o Greedy merge}, and \textit{w/o Operation-specific}.
% }

% =====
\question{
Q8: Discuss multithreaded RTL simulation and whether ARMOR’s compression/code-reuse strategy creates new partitioning, synchronization, or locality challenges.
}

A8: ARMOR is complementary to multithreaded RTL simulation. We have added a discussion in Section 6 explaining that a combined flow can first partition the RTL graph and then apply node compression within each partition. In this way, compressed packs do not cross partition boundaries, introduce no new cross-thread synchronization, and preserve partition-locality.
% The main remaining issue is load balance, since different partitions may expose different compression opportunities and thus have different post-compression workloads. 

% \revision{
% R8: We have added this discussion to Section 6 (Discussion), Complementarity with Parallel Simulation.
% }


% =====
\question{
Q9: Justify the baseline selection and explain why recent simulators such as RTeAAL Sim and GSim are not included.
}

% A9: We have revised Section 5.1 to clarify that our baselines are selected around ARMOR's target setting: cycle-based compiled RTL simulation and front-end/code-footprint reduction. Specifically, we include Verilator, Arcilator, Khronos, Repcut, and RTeAAL Sim as cycle-based compiled RTL simulation baselines, with the RTeAAL Sim results newly added in Figure 9. We also include Dedup and ESSENT because Dedup targets the same front-end bottleneck through code reuse, and ESSENT is its baseline. We do not include GSim because it is an event-driven simulator mainly targeting redundant event optimization, rather than the compiled-code instruction-footprint problem studied by ARMOR.

% A9: We have revised Section 5.1 to clarify that baselines are chosen around ARMOR’s target setting: cycle-based compiled RTL simulation and front-end/code-footprint reduction. We include Verilator, Arcilator, Khronos, Repcut, and the newly added RTeAAL Sim as cycle-based compiled baselines. We also include Dedup because it reduces front-end pressure through code reuse, and ESSENT as Dedup’s baseline. GSim is excluded because it is an event-driven simulator focused on redundant event optimization rather than the compiled-code instruction-footprint problem studied by ARMOR.

A9: We have revised Section 5.1 to clarify that baselines are chosen around ARMOR’s target setting: cycle-based compiled RTL simulation and front-end/code-footprint reduction. We have added RTeAAL Sim as a recent cycle-based simulator baseline, and Figure 9 shows that ARMOR still outperforms it. GSim is excluded because it is an event-driven simulator focused on redundant event optimization rather than the compiled-code instruction-footprint problem studied by ARMOR.


% A9: Our main evaluation focuses on cycle-based compiled RTL simulation, which is ARMOR’s target setting. We do not aim to exhaustively compare with all event-driven simulators. We include Dedup and ESSENT for a specific reason: Dedup is a code-reuse technique for reducing the instruction footprint of compiled RTL simulators, which directly matches the problem ARMOR targets, and ESSENT is Dedup’s baseline. Comparing ESSENT with Dedup also helps expose the limitation of code reuse: although it reduces code footprint, it can introduce additional backend pressure, mainly from indirect memory accesses. 
% In contrast, GSim is an event-driven simulator that mainly focuses on reducing redundant computation, rather than the compiled-code footprint problem studied in ARMOR. 

% We have added RTeAAL Sim as a recent baseline, with results reported in Figure 9.
% In our evaluation, RTeAAL Sim performs comparably to Verilator on CPU designs, consistent with the reported in the original RTeAAL Sim paper, but does not match ARMOR's performance.

% \revision{
% R9: We have revised Section 5.1 to clarify the baseline selection criteria and added the RTeAAL Sim comparison in Figure 9.
% }

% 感觉像是梁云老师审稿的
\subsection{Response to Reviewer \#54B}

\question{
Q1: The authors should discuss whether node compression and multi-threaded partitioning are complementary, and how to choose bit-packing and parallel simulation.
}

A1: ARMOR is complementary to multithreaded RTL simulation. We have added a discussion in Section 6 explaining that a combined flow can first partition the RTL graph using a RepCut-style partitioner and then apply node compression within each partition.

% A1: ARMOR is complementary to multithreaded RTL simulation. A combined flow can partition the RTL graph using the RepCut-style partition algorithm first and then apply node compression within each partition, so compressed packs do not cross partition boundaries, introduce no new cross-thread synchronization, and preserve partition-locality. The main remaining issue is load balance, since different partitions may expose different compression opportunities and thus have different post-compression workloads. 

% \revision{
% R1: We have added this discussion to Section 6 (Discussion), Complementarity with Parallel Simulation.
% }

% \question{
% Q2: Algorithm 2 describes alignment-aware dense node packing at a high level, but the key subroutine SelectMaxFeasibleGroup lacks a detailed description or complexity analysis. Since this is the core packing decision, more details would improve reproducibility.}

\question{Q2: Details of SelectMaxFeasibleGroup in Algorithm 2}

A2: We have revised Section 4.3 to describe "SelectMaxFeasibleGroup". This subroutine is invoked after compression-domain construction and partitioning: the former guarantees structural alignment, while the latter ensures that nodes in each subdomain have no dependencies on each other. Therefore, "SelectMaxFeasibleGroup" selects the largest remaining group from one subdomain that fits in a machine word.

% A2: SelectMaxFeasibleGroup is simple because the compression domain has already enforced the main feasibility constraints. Nodes in the same compression domain are structurally aligned, which means they have the same operation type, operand bitwidths, result bitwidth, and local dataflow structure. Therefore, given a machine-word width \textit{W} and a node slice width \textit{w}, where \textit{w} is the maximum bitwidth among the node’s operands and result, the maximum pack size is floor(\textit{W} / \textit{w}). The subroutine selects up to this many remaining nodes from the domain to form one dense pack. Since \textit{W} is a fixed machine constant, this decision is constant-time per pack, and the total cost over a domain is linear in the number of nodes.

% A2: SelectMaxFeasibleGroup is simple because it is invoked after earlier steps have already made the candidate nodes safe for compression. The compression-domain construction guarantees structural alignment: nodes have the same operation type, operand bitwidths, result bitwidth, and local dataflow structure. Compression-domain partitioning then splits each domain into subdomains, ensuring nodes within each subdomain have no dependencies on each other. 
% Therefore, SelectMaxFeasibleGroup simply selects as many remaining nodes as possible from the subdomain to fill one machine word. 

% \revision{
% R2: We have revised Section 4.3 to add the missing description of SelectMaxFeasibleGroup.
% }

\question{
Q3: Partitioning the compression domain is a non-trivial problem and requires a detailed explanation, because the logic outside the replicated module can change the data dependency of the compression domain. For example: 4 instances F\_1(a\_1, b\_1); F\_2(a\_2, b\_2); F\_3(a\_3, b\_3); F\_4(a\_4, b\_4); have data dependency: a\_1 -> a\_2, a\_3 -> a\_4; would they be completely partitioned, or be partitioned into two (F\_1, F\_2); (F\_3, F\_4) groups?
}

% A3: The reviewer is right that external logic may introduce dependencies among nodes that are initially placed in the same compression domain. ARMOR resolves this before pack construction. A compression domain is a node-level set of structurally aligned nodes, not a group of whole module instances: for each local node in a module definition, ARMOR collects the corresponding nodes across different module instances. Before packing, ARMOR partitions the domain into dependency-free groups (Line 1 in Algorithm 2), ensuring that nodes within groups can be executed in parallel. In the reviewer’s example with dependencies a\_1 -> a\_2, a\_3 -> a\_4, ARMOR would not form instance groups (F\_1, F\_2) and (F\_3, F\_4). Instead, the compression domain \{a\_1, a\_2, a\_3, a\_4\} would be split into dependency-free groups such as \{a\_1, a\_3\} and \{a\_2, a\_4\}, which are executed in dependency order. Thus, no compressed pack contains dependent nodes. 
% A3: In the reviewer’s example, ARMOR would partition the node-level compression domain \{a\_1, a\_2, a\_3, a\_4\} into dependency-free groups such as \{a\_1, a\_3\} and \{a\_2, a\_4\}, rather than forming instance-level groups \{F\_1, F\_2\} and \{F\_3, F\_4\}. This is because a compression domain is not a group of whole module instances, but a node-level set of structurally aligned nodes: ARMOR collects the corresponding nodes across different module instances. ARMOR resolves external dependencies before pack construction by partitioning each compression domain into dependency-free subdomains, as shown in Line 1 of Algorithm 2. Therefore, in this example, ARMOR can partition the compression domain into \{a\_1, a\_3\} and \{a\_2, a\_4\} by using topological order. 
% Thus, no compressed pack contains dependent nodes.

A3: We have added a description of compression-domain partitioning in Section 4.3. In the reviewer's example, ARMOR would not form instance-level groups such as \{F\_1, F\_2\} and \{F\_3, F\_4\}. A compression domain in ARMOR is not a group of whole module instances, but a node-level set of structurally aligned nodes collected across different module instances.  Therefore, ARMOR first constructs the node-level compression domain \{a\_1,a\_2,a\_3,a\_4\}.  If external dependencies exist among these nodes, ARMOR partitions the domain into dependency-free subdomains before pack construction, as shown in Line 1 of Algorithm 2.  In this example, the domain can be partitioned according to topological order into \{a\_1,a\_3\} and \{a\_2,a\_4\}.
% , so each resulting pack remains dependency-free.

% \revision{
% R3: We have added a description of compression-domain partitioning in Section 4.3.
% }

% \question{
% Q4: The core bit-manipulation command, PDEP/PEXT, is not implemented by some CPU generations (for example, AMD Zen 2 doesn’t have dedicated hardware and falls back to a slow microcode routine). The paper should discuss the portability to help the reproduction on different platforms.
% }

\question{
Q4: The paper should discuss the portability of BMI2 to improve reproducibility across different platforms.
}

% A4: We have added a discussion in Section 6 (Portability of BMI2) to clarify this issue. On platforms where PDEP/PEXT is unavailable, ARMOR can fall back to a conservative mode that disables compression for cross-slice-dependent operations while still compressing slice-independent operations.

A4: We have added a portability discussion in Section 6 to clarify that, when PDEP/PEXT is unavailable, ARMOR disables compression for cross-slice dependent operations while still compressing slice-independent ones.

% A4: We agree and have clarified the portability issue. ARMOR uses BMI2 PDEP/PEXT only for cross-slice dependent operations after node compression, such as bit rearrangement. Slice-independent operations, such as AND/OR/XOR/NOT, are still executed using scalar bitwise instructions and do not depend on PDEP/PEXT. Therefore, on platforms where PDEP/PEXT is unavailable, ARMOR can fall back to a conservative mode that disables compression for cross-slice dependent operations while still compressing slice-independent operations. 

% \revision{
% R4: We have added a discussion in Section 6 (Discussion), Portability of BMI2, explaining the role of PDEP/PEXT, the conservative fallback mode.
% }

\question{
Q5: In Section 5.4, the scalability impact is not clear. How does the scalability measured? Are the baselines evaluated by a single thread?
}

% A5: Thank you for pointing out this ambiguity. The “scalability” in Section 5.4 does not refer to host multithreaded scalability. Instead, it measures how the benefit of node compression changes as the amount of module reuse in the RTL design increases. Highly parallel hardware architectures improve architectural parallelism primarily by instantiating multiple identical modules, such as multiple PEs. More module instances usually create more repeated subgraphs, which provide more opportunities for node compression. Therefore, this experiment evaluates whether ARMOR’s compression benefit scales with increasing module reuse/architectural parallelism. All baselines in this experiment are evaluated under the single-thread setting

% \revision{
% R5: We have revised Section 5.4 by clarifying the text to avoid confusing this experiment with host multithreaded scalability. The revised section explicitly states that the experiment measures scaling with module reuse/architectural parallelism.
% }

A5: Thank you for pointing this out. We have revised Section 5.4 to clarify that "scalability" refers to module reuse, not host multithreaded scalability. This experiment evaluates whether ARMOR's performance benefit scales with the degree of module reuse. All baselines are evaluated under the same single-thread setting.

\subsection{Response to Reviewer \#54C:}

We would like to clarify the point "accelerate simulations using the vector instructions" in the paper summary. ARMOR does not rely on vector instructions to implement node compression. Instead, ARMOR packs RTL nodes into bit slices of scalar host machine words and executes them using scalar instructions. 
% ARMOR is complementary to SIMD, and we have clarified this relationship in Section 6 (Relation to SIMD).

\question{
Q1: What is the difference between ARMOR and SLP?
}

{
A1: ARMOR and SLP share the broad idea of exploiting data-level parallelism, but they differ in several high-level aspects:
\begin{itemize}
    % \item \textbf{Different optimization targets.} ARMOR directly targets the generated instruction footprint of compiled RTL simulation and aims to mitigate CPU front-end bottlenecks. SLP primarily targets data-parallel throughput in general-purpose programs by replacing multiple scalar operations with SIMD vector operations. Although SLP may reduce dynamic instruction count, reducing RTL simulator code footprint is not its primary objective.
    \item \textbf{Different optimization targets.} ARMOR directly reduces the generated instruction footprint of compiled RTL simulators to mitigate front-end bottlenecks; SLP may reduce instruction count, but its primary goal is data-parallel throughput in general-purpose programs through auto vectorization.
    % Although SLP may reduce dynamic instruction count, reducing the static instruction footprint of RTL simulators is not its primary objective, and SIMD instructions do not necessarily reduce code footprint.
    \item \textbf{Different execution substrates.} ARMOR uses bit-level parallelism inside scalar host words while SLP uses lane-level parallelism in SIMD registers.
    % \item \textbf{Different optimization stages.} ARMOR is applied at the RTL/FIRRTL lowering stage before C++ code generation, changing the simulator generation strategy from per-node lowering to compressed multi-node lowering. SLP is a compiler optimization applied after scalar code has been generated, typically on compiler IR.
    \item \textbf{Different optimization stages.} ARMOR is applied during RTL-to-C++ lowering, changing simulator generation from per-node lowering to compressed multi-node lowering. In contrast, SLP is applied later on the generated scalar compiler IR.
    % \item \textbf{Different information sources and search spaces.} ARMOR exploits RTL-specific semantic information, such as module hierarchy, to performs module-aware search/alignment on the RTL graph. In contrast, SLP typically starts from local seed packs, often consecutive memory accesses, then expands along use-def/def-use chains within a basic block or local dependence region.
    \item \textbf{Different pack discovery mechanisms.} ARMOR exploits RTL semantics, especially module hierarchy, to perform module-aware subgraph-level search on RTL graphs. In contrast, SLP typically discovers packs by expanding local seeds along dependency chains.
    % \item \textbf{Different execution semantics.} ARMOR provides RTL-operation-specific compressed execution schemes, such as LUT/PEXT/PDEP-based handling for Eq, shift, and bit-extraction operations. SLP generally maps packs to available SIMD operations under specific ISA.
    % \item \textbf{Different lowering mechanisms.} ARMOR lowers compressed packs according to RTL operation semantics and provides operation-specific execution schemes, such as LUT-based execution for Eq groups. In contrast, SLP lowers vector packs to SIMD instructions supported by the target ISA.
    \item \textbf{Different execution optimizations.} ARMOR provides operation-specific execution optimizations, such as LUT-based execution for Eq groups. In contrast, SLP relies on vector instructions provided by the target ISA.
\end{itemize}
}

\question{
Q2: How does ARMOR differ from prior SLP packing and permutation optimizations?
}

% Prior SLP packing and permutation optimizations are closely related, but they address two different subproblems, and ARMOR differs in both.
Prior SLP packing and permutation optimizations are closely related to ARMOR, but ARMOR differs from them.

% \textbf{Pack discovery.} Prior SLP packing methods are largely seed-driven. They usually start from local seed packs exposed in compiler IR, such as consecutive memory accesses, and then expand along use-def/def-use chains within a basic block. ARMOR uses a different, domain-driven approach. Instead of growing packs from local IR seeds, ARMOR first exploits RTL-level semantics, especially structural correspondence across module instances, to construct compression domains. Packing is then performed within these domains under structural-alignment constraints. This is important because RTL graphs often contain many locally isomorphic nodes, and local seed expansion can easily make short-sighted packing decisions, which may introduce excessive data rearrangement in downstream packing. We provide a detailed analysis in Section 3.2.

\textbf{Pack discovery.} Prior SLP packing methods are mostly seed-driven: they start from seeds, such as consecutive memory accesses, and expand along use-def/def-use chains. ARMOR instead packs nodes on top of subgraph-level aligned structures derived from the deterministic correspondence among instances of the same RTL module, rather than relying on local packing decisions. This subgraph-level view helps avoid short-sighted choices that can create excessive downstream data rearrangement; Section 3.3 provides a detailed comparison with local SLP-style packing. Figure 19 (c) shows that the module-aware strategy outperforms the SLP-style strategy, and the supplementary table below further shows that it generally achieves larger average pack sizes with lower data-rearrangement overhead, demonstrating the advantage of module-aware packing.

% \textbf{Permutation Optimization.} For permutation/data rearrangement, the main difference is that ARMOR avoids much of the rearrangement during pack formation, rather than relying on post-packing permutation optimization. Prior SIMD permutation optimizations typically assume that vector packs have already been formed and then try to choose or transform lane orders to reduce shuffle operations between producer and consumer packs. ARMOR instead uses module-aware structural alignment during pack formation: nodes from the same module instance are kept at the same slice position across structurally aligned producer and consumer packs. Therefore, the packed layout can be consistently reused through the isomorphic subgraph, reducing the need for later data rearrangement. This does not mean that ARMOR eliminates all inter-pack rearrangement; however, because structural alignment preserves a consistent slice order across producer-consumer packs, the rearrangement overhead remains moderate and is outweighed by the compression benefit.

% \textbf{Permutation Optimization.} 
% For permutation/data rearrangement, ARMOR reduces rearrangement during pack formation rather than relying mainly on post-packing permutation optimization. Prior SIMD approaches typically form vector packs first and then reduce shuffle operations by choosing or transforming lane orders. ARMOR instead preserves module-aware structural alignment, keeping nodes from the same module instance at consistent slice positions across aligned producer and consumer packs. This lets the packed layout be reused, reducing later rearrangement. 


\textbf{Permutation Optimization.}
ARMOR reduces rearrangement during pack formation rather than relying mainly on post-packing permutation optimization. Prior SIMD approaches typically form vector packs first and then reduce shuffle operations by choosing or transforming lane orders between producer and consumer packs. ARMOR preserves module-aware structural alignment, keeping nodes from the same module instance at consistent slice positions across aligned producer and consumer packs, which reduces pack-to-pack permutation. As shown in the table 2 below, most rearrangement overhead comes from scalar-to-pack formation or pack-to-scalar extraction, rather than permutations between already formed packs.

\begin{table}[h]
\centering
\SetCaptionSpacing{0.10cm}{0.10cm}
\caption{Comparison and breakdown of data-rearrangement overhead.}
\label{tab:rearrangement_breakdown}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|r|r|rrr}
\hline
\multirow{2}{*}{\textbf{Benchmark}} &
\multirow{2}{*}{\textbf{SLP-style}} &
\multirow{2}{*}{\textbf{Module-aware}} &
\multicolumn{3}{c}{\textbf{Module-aware Breakdown}} \\
\cline{4-6}
& & &
\textbf{S$\rightarrow$P} &
\textbf{P$\rightarrow$S} &
\textbf{P$\rightarrow$P} \\
\hline
\hline
Conv2D-16$\times$16    & 30620 & 15532 & 64\% & 27\% & 9\% \\
Gemmini-32$\times$32   & 56971 & 33858 & 47\% & 38\% & 15\% \\
Rocket-8C              & 34829 & 27370 & 57\% & 33\% & 10\% \\
Boom-8C                & 169966 & 165415 & 72\% & 17\% & 11\% \\
\hline
\end{tabular}
}
\vspace{0.5mm}
\begin{flushleft}
\footnotesize
S$\rightarrow$P: scalar-to-pack; P$\rightarrow$S: pack-to-scalar; P$\rightarrow$P: pack-to-pack.
\end{flushleft}
\end{table}



\revision{
% 1. 增加了SLP在RTL graph上做node compression的局限性分析，see xxx
% 2. 增加了消融实验，验证了ARMRO的效果优于SLP，see xxx。
% R2: We have added a detailed analysis in Section 3.3, analyzing the limitations of SLP-style pack discovery on RTL graphs. We also added the "w/o Module-aware" ablation in Section 5.8, showing that ARMOR's module-aware strategy outperforms the SLP-inspired packing strategy.
R2: We added Section 3.3 to compare ARMOR with SLP-style pack discovery on RTL graphs, and Section 5.8.2 includes a "w/o Module-aware" ablation showing the benefit of ARMOR’s module-aware strategy over an SLP-inspired packing strategy.
}

\question{
Q3: Compiler/vectorization evaluation: O2/O3/restrict/AVX
}

% A3: Clang-12 -O2 enables SLP vectorization by default, so our evaluation is conducted with the compiler SLP enabled. 
% To further estimate the effect of compiler optimization and automatic vectorization, 
% We have added a compiler ablation (Section 5.8) using four configurations: O2 without SLP, O2 with SLP, O3 without SLP, and O3 with SLP. The results show that enabling SLP vectorization or increasing the optimization level from O2 to O3 provides only a negligible improvement, indicating that generic compiler vectorization cannot recover the compression opportunities exploited by ARMOR. Regarding restrict, the generated simulator code does not expose the kind of pointer-aliasing ambiguity: most operands are statically generated temporaries or global variables with direct accesses. Section 5.5 does not evaluate SIMD vector widths. It varies ARMOR’s compression granularity, i.e., the maximum number of RTL nodes packed into one scalar machine word. 
% ARMOR’s current implementation uses scalar-word bit-slice execution rather than SIMD vector lanes. We clarify the relationship between ARMOR and SIMD in Section 6, where we discuss SIMD as a complementary backend for future wider compressed execution.

% A3: Clang-12 -O2 enables SLP vectorization by default, so our evaluation is conducted with the compiler SLP enabled. We further added a compiler ablation in Section 5.8 with four configurations: O2/O3 with and without SLP. The results show that enabling SLP vectorization or increasing the optimization level from O2 to O3 provides only a negligible improvement, indicating that generic compiler vectorization cannot recover the compression opportunities exploited by ARMOR. Regarding restrict, the generated simulator code does not expose the kind of pointer-aliasing ambiguity: most operands are statically generated temporaries or global variables with direct accesses. Section 5.5 does not evaluate SIMD vector widths. It varies ARMOR’s compression granularity, i.e., the maximum number of RTL nodes packed into one scalar machine word. 

A3: Clang-12 -O2 enables SLP vectorization by default, so our evaluation is conducted with the compiler SLP enabled. We further added a compiler ablation in Section 5.8.1 with four configurations: O2/O3 with and without SLP. The results show that enabling SLP or increasing the optimization level brings negligible improvement, indicating that generic compiler vectorization cannot recover RTL-specific compression opportunities. We did not separately evaluate restrict, because ARMOR-generated code primarily uses statically generated temporaries and direct accesses to global variables, rather than pointer-heavy code with ambiguous aliasing; we therefore do not expect restrict to materially affect the results. Finally, ARMOR currently does not use AVX or AVX2. Section 5.5 varies the maximum number of RTL nodes packed into one scalar machine word, not the SIMD vector width.

\revision{
R3: We have added a compiler ablation study in Section 5.8.1.
% and revised Section 6 to clarify that ARMOR currently uses scalar-word bit-slice execution while SIMD is complementary.
}

\question{
Q4: Slice-Dependent Operations vs. SIMD Horizontal Operations}

% A4: SIMD horizontal operations and ARMOR’s slice-dependent operations both involve cross-lane or cross-slice interactions, but the source and role of such interactions are fundamentally different. In SIMD horizontal operations, cross-lane dependence is the intended semantics of the operation. For example, horizontal add or dot product explicitly combines values from multiple SIMD lanes to produce a reduction or aggregate result. The cross-lane is therefore the computation that the SIMD instruction is designed to perform.
% In ARMOR’s bit-level packing, however, different slices represent independent RTL nodes or bit fields. Ideally, each slice should be computed only from its corresponding input slice and should not be affected by other slices. Cross-slice dependence appears only because multiple slices are packed into the same host word, and some word-level operations may accidentally propagate information across slice boundaries, such as aggregation in Eq operations or boundary crossing in shifts/extractions. These cross-slice effects are not part of the original RTL semantics; they are side effects introduced by packed host-word execution.
% Therefore, SIMD horizontal operations aim to exploit intended cross-lane computation, whereas ARMOR’s handling of slice-dependent operations aims to identify, isolate, or eliminate unintended cross-slice interference so that each packed slice still correctly simulates its corresponding RTL node.

% A4: SIMD horizontal operations and ARMOR's slice-dependent operations both involve cross-lane or cross-slice interactions, but their intent different. In SIMD horizontal operations, cross-lane dependence is the intended semantics: operations such as horizontal add or dot product explicitly combine values from multiple lanes to produce a reduction or aggregate result. In ARMOR, different bit slices represent independent RTL nodes, so each slice should ideally depend only on its corresponding input slice. Cross-slice dependence appears only because multiple slices are packed into the same host word, where some word-level operations may unintentionally propagate information across slice boundaries. Therefore, ARMOR’s handling of slice-dependent operations aims to eliminate unintended cross-slice interference to preserve correct per-slice RTL semantics.


A4: SIMD horizontal operations intentionally introduce cross-lane aggregation, whereas ARMOR's slice-dependent operations must avoid unintended cross-slice interference. In SIMD, operations such as the dot product explicitly combine values from multiple lanes to produce an aggregate result. In ARMOR, different bit slices represent independent RTL nodes, so cross-slice dependence is not part of the intended RTL semantics; it only arises from packing multiple slices into the same host word. Therefore, ARMOR handles slice-dependent operations to preserve correct per-slice semantics.

\subsection{Response to Reviewer \#54D:}

\question{
% Q1: Alg 1. uses names to identify the nodes that can be packed together. This may be another artifact of the two representations (see below), but once you get to the module level, isn't the number of operations small enough that a proper graph isomorphism algorithm is not prohibitively expensive?
Q1: Once you get to the module level, isn't the number of operations small enough that a proper graph isomorphism algorithm is not prohibitively expensive?
}

% A1: We would like to clarify that name-based alignment is not a representation artifact, but an efficiency-oriented design choice. 
% Node names are unique within a module definition, so the same module-scoped node name in different instances naturally identifies corresponding nodes.
% For a single small module-level subgraph, a graph-isomorphism algorithm may be affordable; however, ARMOR needs to perform matching across a large number of module instances, where repeatedly invoking a general graph-isomorphism algorithm would become expensive. 
% Although graph-isomorphism matching may be affordable for a module-level subgraph, repeatedly applying it across many module instances would be costly.
% Thus, ARMOR uses module-aware name alignment as an efficient alternative.



A1: We would like to clarify that name-based alignment is not a representation artifact, but an efficiency-oriented design choice. Although graph-isomorphism matching may be affordable for a module-level subgraph, repeatedly applying it across many module instances would be costly.

\question{
Q2: Alg 2. It is not clear from the algorithm that UPDATE(N, PN) removes node N from N.domain. Providing a specification for that function would be helpful.
}

A2: We have revised Algorithm 2 by replacing UPDATE(N, P\_N) with the explicit statements “remove P\_N from N.domain” and “insert P\_N into N.packs” avoiding ambiguity about the update behavior.

\question{
Q3: I did not follow how the LUT-based compression execution for Eq operations works: it seems to require the range of values for both the non-const operand and the const operand. Where does ARMOR retrieve these values from?
}

% A2: The required values are obtained from two sources. First, the value range is known at compile time from the bitwidth of the operands, so ARMOR can determine the LUT size during code generation. Second, for an Eq group of the form x == c\_i, the constant operands c\_i are literals extracted from FIRRTL at compile time, while the non-constant operand x is a runtime value. In the LUT-based execution, each constant c\_i corresponds to a LUT entry, and the runtime value of x is used as the LUT index. Since all Eq operations in the group share the same x, at most one Eq result is true at a time. Therefore, when x changes from an old value to a new value, ARMOR resets the LUT entry indexed by the old value and sets the entry indexed by the new value. The result of each Eq operation x == c\_i is then obtained by reading the LUT entry associated with the compile-time constant c\_i; PEXT can be further used to extract multiple such Eq results in parallel.

A3: The required values come from compile-time FIRRTL metadata and runtime operand. For an Eq group of the form (x == c\_i), the bitwidth of the shared non-constant operand (x) determines the value range and hence the LUT size. The constants (c\_i) are FIRRTL literals known at compile time, while (x) is a runtime value used as the LUT index. At each simulation cycle, ARMOR updates the LUT by clearing the entry indexed by the old value of (x) and setting the entry indexed by the new value. Each Eq result (x == c\_i) is then obtained by reading the LUT entry indexed by (c\_i). A detailed description of the LUT-based execution is provided in Section 4.4.4.


\revision{
R3: We have revised Section 4.4.4 to clarify the source of the values used in LUT-based Eq execution. 
% The revised text states that Eq groups consist of a shared non-constant operand whose value is produced at runtime and compile-time constant literals. It also clarifies that the LUT size is determined by the bitwidth of operands, whose value range is known at compile time.
}


\question{
% Q4: throughout the paper there are discussions on the front-end bottlenecks and L1 cache pressure. Indeed, the resulting code exceeds the cache capacity, but unless there is code reuse, the L1 cache will miss unless prefetching can keep up with the execution. I did not see any data in the paper discussing how much code reuse there is.
Q4: How much code reuse is there?
}

A4: ARMOR does not implement explicit function-level code reuse by factoring repeated RTL nodes into a shared function. Instead, node compression creates implicit instruction-sequence reuse: one compressed instruction sequence represents the scalar execution of multiple isomorphic RTL nodes. We have added Figure 11 and the corresponding analysis in Section 5.2 to quantify this reuse using the eliminated-instruction percentage relative to scalar per-node lowering. The results show that ARMOR reduces the generated static instruction footprint by 29.4\% on average.

% A4: ARMOR does not implement explicit code reuse by factoring repeated RTL nodes into a shared function and invoking it repeatedly. Instead, ARMOR creates implicit code reuse at the instruction-sequence level: one instruction sequence represents the scalar execution of multiple isomorphic RTL nodes. To quantify this implicit code reuse, we added a new experiment using the eliminated instruction percentage relative to scalar per-node lowering. ARMOR achieves an average static implicit code reuse rate of 29.4\% (up to 56.78\%), meaning that 29.4\% of the generated instruction footprint is reduced by reuse. 
% The result shows that node compression provides substantial instruction-sequence reuse, thus reducing the instruction footprint and alleviating L1I pressure.
% From the dynamic-execution perspective, ARMOR achieves an average dynamic implicit code reuse rate of 24.54\% (up to 51.16\%), meaning that 24.54\% of dynamically executed scalar instructions are avoided through compressed execution. These results show that node compression provides substantial instruction-sequence reuse, directly reducing the instruction footprint and alleviating L1I pressure.

\revision{
R4: We have added Figure 11 and the corresponding analysis in Section 5.2. 
}

\question{
Q5: I disagree with the claim that SIMD is different. Yes, one may look at the vector units as coarse-grained, but you can also consider them as 512-bit machine words. Why is node-compression limited to the "fine-grained" 64 bits? 
}

A5: We agree that SIMD registers can be viewed as wider bit containers, and node compression is not fundamentally limited to 64-bit scalar words. In ARMOR, the 64-bit scalar word is an implementation substrate, not a conceptual limitation. ARMOR currently uses scalar-word bit-slice execution, while using SIMD/vector units as a wider backend for node compression is an interesting direction for future work.


% A5: We agree that SIMD registers can be viewed as wider bit containers, and node compression is not fundamentally limited to 64-bit scalar words. The current 64-bit scalar word is an implementation substrate, not a conceptual limitation. The  difference is not the physical register width, but the exposed operation model. SIMD instructions typically operate on ISA-defined homogeneous element lanes, such as 8-, 16-, 32-, or 64-bit elements, whereas ARMOR uses software-defined bit slices whose widths are determined by the actual RTL node bitwidths. Since RTL nodes often have narrow, irregular, or mixed bitwidths, directly mapping them to SIMD lanes can still waste bits or require extra packing/unpacking, masks, and shuffles.
% ARMOR currently uses scalar words because ordinary bitwise operations and BMI2 PDEP/PEXT provide direct fine-grained control over bit-slice layout. This makes scalar-word execution a simple and efficient backend for our first implementation. SIMD and ARMOR are therefore complementary rather than mutually exclusive: ARMOR can first perform bit-level node compression, and future backends could use SIMD registers to process multiple compressed words or implement wider packs.

\revision{
R5: We have revised Section 6 to clarify that the 64-bit scalar word is an implementation substrate rather than a conceptual limitation. 
% The revision explains the difference between SIMD’s ISA-defined homogeneous lanes and ARMOR’s software-defined bit slices, and states that SIMD and ARMOR are complementary.
}

\question{
Q6: Writing-related.
}

A6: Thank you for the writing-related comments. We have rewritten Section 3.3 to improve clarity and readability.

\question{
% Q7: I do not understand what is the relevance of section 2.2, especially the first paragraph where you discuss data-center scale profiling
Q7: Relevance of Front-End Background in Section 2.2.
}

A7: Section 2.2 is intended to provide a brief background on the CPU front-end and related hardware-side mechanisms for mitigating front-end bottlenecks. We have removed the original data-center-scale profiling discussion.

\question{
Q8: It would be nice to add Arcilator as a comparison point. It compiles CIRCT IR directly, and it tends to be faster than Verilator.
}

A8: We have added Arcilator to Figure 9. Although Arcilator outperforms Verilator on AI accelerators and is comparable on CPU cores, ARMOR still achieves the best performance.


\subsection{Response to Reviewer \#54E:}


\question{
Q1: Can the authors add or discuss results on lower-reuse or more irregular RTL designs to clarify when node compression becomes less effective?
}

% A1: We agree that ARMOR’s benefit depends on the amount of structural reuse in the RTL design, and lower-reuse or more irregular designs are less favorable cases. 
% Section 5.4 studies this factor by varying the number of replicated module instances. The results show the expected trend: for the Conv2D design, the speedup over Repcut improves from 1.46$\times$ under the 2$\times$2 PE array to 4.63$\times$ under the 20$\times$20 PE array. This indicates that node compression becomes less effective as module reuse decreases.
% However, modern accelerators and multicore designs increasingly rely on replicated modules, making ARMOR valuable for exploiting such structural regularity.

% \revision{
% R1: We have revised Section 5.4 and added a discussion clarifying that highly irregular RTL with little module reuse is expected to benefit less from node compression.
% }

% A1: Section 5.4 studies ARMOR's performance benefit scales with the degree of module reuse. The results show the expected trend: node compression becomes less effective as module reuse decreases. However, modern accelerators and multicore designs increasingly rely on replicated modules, making ARMOR valuable for exploiting such structural regularity.

A1: Section 5.4 studies how ARMOR’s benefit changes with module reuse. As expected, node compression becomes less effective when module reuse decreases, but modern accelerators and multicore designs often use replicated modules, where ARMOR can exploit the resulting structural regularity.

\question{
Q2: Can the authors better position the novelty relative to prior bit-parallel/SWAR-style simulation and module-reuse/code deduplication techniques?
}

% A2: We agree that bit-level/SWAR-style execution, repeated-structure exploitation, and code-footprint reduction each have prior analogues. ARMOR’s novelty is not claiming any of these ingredients in isolation. Rather, ARMOR identifies a specific opportunity in compiled RTL simulation: fully unrolled RTL graphs expose many structurally aligned low-bitwidth nodes, while per-node lowering wastes machine-word bit space and creates excessive instruction footprint. ARMOR turns this observation into an automatic RTL node-compression framework, combining module-aware isomorphic subgraph identification, alignment-aware packing, and RTL-operation-specific compressed execution, thereby reducing the generated instruction footprint and alleviating the front-end bottleneck in RTL simulation. Compared with SWAR-style techniques, ARMOR is not only a low-level bit-packing idiom, but an end-to-end RTL-level framework that automatically discovers, packs, and executes compressible RTL nodes. Compared with module-reuse/code-deduplication techniques, ARMOR uses module hierarchy to find node-level structural alignment rather than extracting repeated modules into explicit reusable functions, thereby preserving the fully unrolled, statically specialized simulation substrate.

% A2: ARMOR's novelty lies in identifying a new opportunity in fully unrolled compiled RTL simulation: many structurally aligned, low-bitwidth RTL nodes are lowered independently, wasting machine-word bit space and inflating the generated instruction footprint. ARMOR exploits this opportunity through node compression: it uses module hierarchy to identify node-level structural alignment, packs aligned nodes into machine-word slices, and lowers them with RTL-operation-specific execution schemes. 
% Compared with SWAR-style techniques, ARMOR is not only a low-level bit-packing idiom, but an end-to-end RTL-level framework that automatically discovers, packs, and executes compressible RTL nodes. 
% Compared with code-deduplication techniques, ARMOR preserves the fully unrolled, statically specialized simulation substrate instead of factoring repeated logic into shared functions.

% A2: ARMOR's novelty lies in identifying a new opportunity in fully unrolled compiled RTL simulation: many structurally aligned, low-bitwidth RTL nodes are lowered independently, wasting machine-word bit space and inflating the generated instruction footprint. ARMOR exploits this opportunity through node compression. Compared with SWAR-style techniques, ARMOR is not only a low-level bit-packing idiom, but an end-to-end RTL-level framework that automatically discovers, packs, and executes compressible RTL nodes. Compared with code-deduplication techniques, ARMOR preserves the fully unrolled, statically specialized simulation substrate instead of factoring repeated logic into shared functions.

A2: ARMOR’s novelty is identifying a new opportunity in fully unrolled compiled RTL simulation: many structurally aligned, low-bitwidth RTL nodes are lowered independently, wasting machine-word bit space and inflating instruction footprint. ARMOR exploits this opportunity through node compression. Unlike SWAR-style bit-packing idioms, ARMOR is an end-to-end RTL-level framework that automatically discovers, packs, and executes compressible nodes. Unlike code deduplication, ARMOR reduces footprint while preserving the fully unrolled, statically specialized simulation substrate instead of factoring repeated logic into shared functions.

\question{
Q3: Why is a general automatic framework needed instead of targeted/manual component-level bit-packing optimizations?
}

% A3: RTL simulators are core chip-design infrastructure and are typically used as black-box tools by hardware designers, who should not need to reason about compiler-level code generation to obtain fast simulation. 
% ARMOR keeps the RTL unchanged and automatically performs node compression during simulator generation, making bit-level packing design-independent and transparent to RTL designers.


A3: RTL simulators are core chip-design infrastructure and are typically used as black-box tools, so hardware designers should not need to manage compiler-level code generation for performance. ARMOR keeps the RTL unchanged and automatically applies node compression during simulator generation, making the optimization transparent to users.

